TARJAMAT: Evaluation of Bard and ChatGPT on Machine Translation of Ten Arabic Varieties

Despite the purported multilingual proficiency of instruction-finetuned large language models (LLMs) such as ChatGPT and Bard, the linguistic inclusivity of these models remains insufficiently explored. Considering this constraint, we present a thorough assessment of Bard and ChatGPT (encompassing both GPT-3.5 and GPT-4) regarding their machine translation proficiencies across ten varieties of Arabic. Our evaluation covers diverse Arabic varieties such as Classical Arabic (CA), Modern Standard Arabic (MSA), and several country-level dialectal variants. Our analysis indicates that LLMs may encounter challenges with dialects for which minimal public datasets exist, but on average are better translators of dialects than existing commercial systems. On CA and MSA, instruction-tuned LLMs, however, trail behind commercial systems such as Google Translate. Finally, we undertake a human-centric study to scrutinize the efficacy of the relatively recent model, Bard, in following human instructions during translation tasks. Our analysis reveals a circumscribed capability of Bard in aligning with human instructions in translation contexts. Collectively, our findings underscore that prevailing LLMs remain far from inclusive, with only limited ability to cater for the linguistic and cultural intricacies of diverse communities.

==> Sections/Lit_Review/karimaLit.tex <==
\subsection{Karima Related Work}\label{sec:karimaRel}

In their efforts to maximize ChatGPT's translation aptitude, \cite{peng2023making} tested temperature adjustment and specifying task and domain information on different pairings of English, German, Romanian and Chinese. 
They found that lower temperature values generally led to better performance, with a value of 0 being adopted. 
By starting the prompt with the sentence: \textit{"You are a machine translation system in the [DOM] domain"} the authors saw an increased performance, possibly attributed to (1) decreasing the gap between the conversation and translation objectives (which is an important difference between Large Language Models (LLMs) and Neural Machine Translation (NMT) systems) and (2) leveraging ChatGPT's cross-domain generalization capability. 
Although hallucinations were witnessed with non-English-centric language pairs, they could be mitigated using lower temperatures and task-specific prompts. 
Few-shot In-Context Learning (ICL) \cite{icl} and Chain-of-Thought (CoT) \cite{cot} were also explored. ICL proved to improve performance on both BLEU \cite{bleu} and COMET \cite{comet}, although increasing the number of shots above 1 did not yield better results. On the other hand, performance worsened with CoT, causing word-by-word translation.

In \cite{hendy2023good}, the effectiveness of GPT 3.5 was studied in sentence-level and document-level translation, in addition to its ability to generalize across domains. They used a range of 18 languages from the WMT22 and WMT21 datasets.
For high-resource languages, GPT 3.5 demonstrated remarkable zero-shot performance when translating into English, with no notable few-shot improvement. It outperformed both WMT-Best \cite{wmt22} and Microsoft-Translator for German, Japanese, and Chinese. 
When translating from English, few-shot settings outperformed zero-shot particularly when using a single high-quality shot (determined by cosine distance between the LaBSE \cite{labse} embeddings of the shot and the input sentence). 
When it comes to low-resource languages, some modest gains were observed with a single high-quality shot but not enough to surpass WMT-Best for any language. The single shot was also beneficial for non English-centric translations, allowing the model to translate into the appropriate language better. Both the zero-shot and single-shot configurations outperform the commercial systems on the COMET metric.
For all languages, however, an important and steady degradation is witnessed on lexical metrics (BLEU and ChrF \cite{chrf}). 
Experiments showed that document-level translation surpassed the equivalent sentence-level ones, with no significant few-shot improvement. This suggests that the document context already supplies sufficient information, making additional shots dispensable for document-level translation.
Finally, the authors report good translation robustness when evaluating on different domains (namely social, news, conversational and e-commerce) despite some inconsistency on lexical metrics for the German and Chinese languages on the social and news domains.



==> Sections/Lit_Review/samarLit.tex <==
\subsection{Samar Related Work}\label{sec:samarRel}
Recently, ChatGPT has received a great deal of attention, especially since the release of its premium version, ChatGPT 4. Many researchers examined ChatGPT's capabilities as an MT tool compared with other commercial translation products. Jiao et al., 2023 \cite{jiao2023chatgpt} conducted a preliminary evaluation of ChatGPT as an MT model by comparing its translation output with three commercial translation products, namely Google Translate, DeepL Translation, and Tencent TranSmart). These products support translation in 133,29 and 16 languages. The study included translation prompts, multilingual translation, and translation robustness. In the study, the prompts were generated by ChatGPT as recommendations to trigger the best prompts for minor performance differences. They consider that this study's results date back to ChatGPT version 2022.12.16. 

Data used in this study for multilingual translation include the Flores 101 test set, which consists of 1012 sentences translated into 101 languages. To test ChatGPT's translation robustness, they used the WMT19 Biomedical Translation Task test set (Bawden et al., 2019). Also, set 2 and set 3 of the MWT20  Robustness Task (Specia et al., 2020, i.e., Rob2 and Rob3). Regarding the evaluation metric, the study by Jiao et al. employed BLUE Score as the primary metric and report Chrf++ and TER. The study developed an effective strategy called pivot prompting in which they ask ChatGPT to translate the source language into a high-resource pivot language before translating it into the target language. They claim that this strategy improves translation performance significantly. The study concluded that ChatGPT performs competitively with chimerical products (Google Translate, DeepL Translate, and Tencent TranSmart) when evaluating its performance on the benchmark mentioned above test sets, especially in high-resource European languages. However, its ability lags behind low-resource or distant languages. On the robustness level, ChatGPT doesn't perform as well as commercial systems in biomedical abstracts and Reddit comments. Nevertheless, ChatGPT exhibits good results in spoken language. The study inferred that ChatGPT had become a good translator in terms of performance compared to other commercial translation products, even for distant languages. 

Providing the appropriate prompts is an effective way to get the ultimate performance of ChatGPT. Therefore, prompts play a crucial role in unleashing ChatGPT's translation abilities. According to \cite{gao2023design}(Gao et al.2023), to get the highest results out of ChatGPT's translation performance, one needs to use suitable prompts. This study offers several translation prompts that include: translation task information (e.g., English into German), context domain information (e.g., News), and parts of speech (POS) tags, which help unleash ChatGPT's translation abilities. 
The study concludes that ChatGPT achieves better results than commercial translation systems only when using the appropriate prompts. Goa employed the multi-inference test set to evaluate ChatGPT performance, indicating that translation performance significantly differs from the single reference evaluation. 




==> Sections/datasets_prev.tex <==
\section{Datasets}\label{sec:data}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Translation Datasets}\label{subsec:transData}

In order to evaluate ChatGPT's ability to translate from different varieties of Arabic, we collect data as follows:

\subsubsection{Arabic Varieties Translation}
\begin{itemize}
    \item \textbf{CA:} We collect a total of 200 sentences from the OpenITI \cite{nigst2020openiti} dataset. The sentences are drawn from various books that belong to the second century AH. The selected sentences demonstrate the CA's distinct linguistic features regarding word richness, semantic variations, and the usage of Tashkeel.
    % Each sentence is at least ten words long. 
    \item \textbf{MSA:} We collect a total of 200 sentences from current events news from two online news websites:
    % 50 from each of 
    \href{https://aljazeera.net/news}{Aljazeera} and \href{https://bbc.com/arabic}{BBC Arabic}. The curated sentences showcase various news genres, including political, social, and sports, among others.
    % The length of the sentence is not less than ten words each. 
    \item \textbf{DA:} We manually collect a dataset of Dialectal Arabic collected from an in-house project where we transcribe TV series collected from YouTube videos belonging to Arabic dialects. In this paper, we focus on the following dialects:
    \begin{itemize}
        \item Algerian (ALG)
        \item Egyptian (EGY)
        \item Emirati (UAE)
        \item Jordanian (JOR)
        \item Mauritanian (MAU)
        \item Moroccan (MOR)
        \item Palestinian (PAL)
        \item Yemen (YEM)
    \end{itemize}
    1600 sentences are chosen, 200 from each, to test ChatGPT's abilities on the dialectal level. 
    % \item \textbf{MWEs:} We collected 100 sentences of verbal MWEs in Modern Standard Arabic from \cite{mohamed2022annotating} the PARSEME dataset.
    % \item \textbf{Syntactic Ambiguity:} One of the linguistic features we are testing is ChatGPT's ability to translate syntactic ambiguous sentences in Arabic. We collected 40 MSA ambiguous sentences from different theses tackling this feature in the Arabic language. 
    % \item \textbf{Collocations:} 
    % \item \textbf{Proverbs:} We selected a hundred proverbs in MSA from websites teaching Arabic as a foreign language. 
    % 150 Egyptian proverbs are collected from websites teaching Egyptian Arabic to non-natives and their meanings in English. 
    % \todo{add MOR}
    % Examples of these proverbs are provided in Table \ref{tab:proverb_examples}.
    % \item \textbf{Synonyms and Antonyms:} To test ChatGPT's linguistics abilities in understanding synonyms and antonyms, 50 words in Egyptian and Moroccan dialects are selected from \cite{abdul2020dialex} Dialex dataset for dialectal Arabic word embedding and the Darija Open Dataset (DODa) respectively \cite{outchakoucht2021moroccan} \todo{Review section after word selection is done}. 
    % \item \textbf{Hypernyms and Hyponyms} In order to test ChatGPT's lexical capabilities in Egyptian and Moroccan dialects, we curated 50 words from \cite{abdul2020dialex}. When selecting nouns, we tend to choose words that are not code-switched or borrowed and incorporate a wide range of hyponyms. 
\end{itemize}
Each sentence in the above datasets is at least 10 words long. 
% The selected DA sentences are free of code-switching. \todo{Make sure this is the case for all DAs}
Table \ref{tab:variety_examples} shows two examples from each of these datasets.

% \begin{landscape}
\begin{table*}[t]
    \centering
    \begin{tabular}{|c|p{0.4 \linewidth}|p{0.4\linewidth}|}
    % \begin{tabular}{|c|p{0.5 \linewidth}|p{0.5 \linewidth}|}
    \hline
    Variety & Examples & English Translation\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    MSA & \RaggedRight{\begin{arabtext} \small اكتسح مانشستر سيتي مضيفه ساوثهامبتون 4-1 اليوم السبت ضمن منافسات الجولة 30 من الدوري الإنجليزي لكرة القدم. \end{arabtext}} & On this Saturday, Manchester City swept Southampton 4-1, in the 30th round of the English Premier League.\\ 
    % \multirow{2}{*}{MSA} & \RaggedRight{\begin{arabtext} \small اكتسح مانشستر سيتي مضيفه ساوثهامبتون 4-1 اليوم السبت ضمن منافسات الجولة 30 من الدوري الإنجليزي لكرة القدم. \end{arabtext}} & On this Saturday, Manchester City swept Southampton 4-1, in the 30th round of the English Premier League.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small شهدت أسهم البنوك حول العالم تراجعا حادا وسط مخاوف من تعرّض بنوك أخرى لمشكلات مشابهة، ومن اندفاع المستثمرين إلى سحب أموالهم.\end{arabtext}} & Bank stocks around the world witnessed a sharp decline amid fears that other banks would be exposed to similar problems, and that investors would rush to withdraw their money.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    CA & \RaggedRight{\begin{arabtext} \small وكانت بنو مليح من خزاعة وهم رهط طلحة الطلحات يعبدون الجن\end{arabtext}} & Banū Malī\d{h}, Raht Tal\d{h}aht El-Tal\d{h}at, tribe which descended from Khuza'ah tribe, used to worship Jinn.\\ 
    % \multirow{2}{*}{CA} & \RaggedRight{\begin{arabtext} \small وكانت بنو مليح من خزاعة وهم رهط طلحة الطلحات يعبدون الجن\end{arabtext}} & Banū Malī\d{h}, Raht Tal\d{h}aht El-Tal\d{h}at, tribe which descended from Khuza'ah tribe, used to worship Jinn.\\ 
    % \cline{2-3}
    % &  \RaggedRight{\begin{arabtext} \small فغاية الناس وحاجاتهم صلاح المعاش والمعاد، والسبيل إلى دركها العقل الصحيح.\end{arabtext}} & The ultimate goal or need that people seek is creating a better life and afterlife; and common sense is the only means to reach them.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    ALG & \RaggedRight{\begin{arabtext} \small   \end{arabtext}} & \\ 
    % \multirow{2}{*}{ALG} & \RaggedRight{\begin{arabtext} \small   \end{arabtext}} & \\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small \end{arabtext}} & \\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    EGY & \RaggedRight{\begin{arabtext} \small ماحنا لو فضلنا مدارين و مستخبين هنموت من الخوف. \end{arabtext}} & And if we keep hiding, we’re going to die out of fear.\\ 
    % \multirow{2}{*}{EGY} & \RaggedRight{\begin{arabtext} \small ماحنا لو فضلنا مدارين و مستخبين هنموت من الخوف. \end{arabtext}} & And if we keep hiding, we’re going to die out of fear.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small طب اقعد أعمل كوبيتين شاي من بتوع زمان و نقعد ندردش براحتنا. \end{arabtext}} & Just go make some tea, tea of the old days, so we can chill and talk\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    JOR & \RaggedRight{\begin{arabtext} \small   أنا مش مستخف فيه و لا يمكن استخف فيه مهما كان بضل ابوي\end{arabtext}} & I do not and cannot underestimate him; he is still my father, no matter what.\\ 
    % \multirow{2}{*}{JOR} & \RaggedRight{\begin{arabtext} \small   أنا مش مستخف فيه و لا يمكن استخف فيه مهما كان بضل ابوي\end{arabtext}} & I do not and cannot underestimate him; he is still my father, no matter what.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small لا فترة قصيرة ولا اشي، أنا صارلي عايشه بينهم اكثرمن شهرين وأظن هالفترة كافية مشان اعرف عنهم كل اشي\end{arabtext}} & It is not a short time. Having lived with them for over two months, I feel that I have sufficient time to become familiar with every aspect of their lives.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    MAU & \RaggedRight{\begin{arabtext} \small   شوف آن شي كامل ادخلتو ماتيت انركيلي فيه خالك اللا القدام.\end{arabtext}} & Look, whenever I'm in, I never take a step back; I only go forward.\\ 
    % \multirow{2}{*}{MAU} & \RaggedRight{\begin{arabtext} \small   شوف آن شي كامل ادخلتو ماتيت انركيلي فيه خالك اللا القدام.\end{arabtext}} & Look, whenever I'm in, I never take a step back; I only go forward.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني انو بدو يبقى ياران لك ملي ما فايتن علنك ما تيت تقعد هون في البوتيك\end{arabtext}} & For your record, we are aware that you no longer sit with us in the store.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    MOR & \RaggedRight{\begin{arabtext} \small بحالا علمك الله آ سي علي. شفت كلشي. و دابا را كلشي ولا باين و ما بقى ما يتخبى.\end{arabtext}} & It's as though God warned you, Mr. Ali. I saw everything. And now everything became clear and there is nothing to hide anymore\\ 
    % \multirow{2}{*}{MOR} & \RaggedRight{\begin{arabtext} \small بحالا علمك الله آ سي علي. شفت كلشي. و دابا را كلشي ولا باين و ما بقى ما يتخبى.\end{arabtext}} & It's as though God warned you, Mr. Ali. I saw everything. And now everything became clear and there is nothing to hide anymore\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small لا لا، جيت هي نشوف نادية على شي غرض. بغيت غي نسولها على شي حاجة.\end{arabtext}} & No, no. I just came to see Nadia for something. I just want to ask her about something.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    PAL & \RaggedRight{\begin{arabtext} \small   يا رب هالاجتماع يخلص بسرعة لأنه عمي أبو العبد اذا بضل يفوتلنا من قصة و يطلعلنا من قصة الكلاسيكو بروح علينا.\end{arabtext}} & God I hope this meeting ends quickly because if uncle Abu al Abed keeps rambling we will miss the Classico.\\ 
    % \multirow{2}{*}{PAL} & \RaggedRight{\begin{arabtext} \small   يا رب هالاجتماع يخلص بسرعة لأنه عمي أبو العبد اذا بضل يفوتلنا من قصة و يطلعلنا من قصة الكلاسيكو بروح علينا.\end{arabtext}} & God I hope this meeting ends quickly because if uncle Abu al Abed keeps rambling we will miss the Classico.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني انو بدو يبقى يا سيدي، معقول شرطة من الداخلية أو سيارة شرطة هيك عابرة سبيل؟.\end{arabtext}} & So who could it be sir, could it be a police from the ministry of the interior or just a police car passing by?\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    UAE & \RaggedRight{\begin{arabtext} \small لا أنا ما قلت جيه يالياسمينه أنا أقول إن راجح مسوي هالخطة عشان يزخ الحرامي.\end{arabtext}} & No, Yasmina, I did not say that. I'm saying Rajah devised this plan to capture the thief.\\ 
    % \multirow{2}{*}{UAE} & \RaggedRight{\begin{arabtext} \small لا أنا ما قلت جيه يالياسمينه أنا أقول إن راجح مسوي هالخطة عشان يزخ الحرامي.\end{arabtext}} & No, Yasmina, I did not say that. I'm saying Rajah devised this plan to capture the thief.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small ان شاء الله ان شاء الله يا عمي، أنا بس يعني أبغى أخبرك، أقولك شو استوى في الفريج.\end{arabtext}} & God willing, uncle God willing, I just wanted to let you know what happened in the neighborhood.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    YEM & \RaggedRight{\begin{arabtext} \small   ركزت لي نفطة تفتيش، في الباب، بتفتش ذي داخلي و ذي خارجي.\end{arabtext}} & I set up a checkpoint at the door to screen anyone who comes in or out.\\ 
    % \multirow{2}{*}{YEM} & \RaggedRight{\begin{arabtext} \small   ركزت لي نفطة تفتيش، في الباب، بتفتش ذي داخلي و ذي خارجي.\end{arabtext}} & I set up a checkpoint at the door to screen anyone who comes in or out.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني ابي و ابوش هكذا عيجلسوا محبوسين و نحنا نجلس نتفرج.\end{arabtext}} & This means that both my father and your father will be imprisoned, and we will be powerless to intervene.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}
    \caption{Example sentences from each of the Arabic varieties in the translation datasets. MSA: Modern Standard Arabic. CA: Classical Arabic. EGY: Egyptian Dialect. MOR: Moroccan Dialect}
    \label{tab:variety_examples}
\end{table*}
% \end{landscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Multi-Word Expressions Translation}
We collected 100 sentences of verbal MWEs in Modern Standard Arabic from the PARSEME dataset \cite{mohamed2022annotating}.
\todo{Define MWEs (+ diff w/ collocs) + selection criteria if any + we translated them professionally}
Table \ref{tab:mwe_examples} shows examples of said MWEs with their English translations.

\begin{table*}[t]
    \centering
    \begin{tabular}{|p{0.5\linewidth}|p{0.5\linewidth}|}
    \hline
    MSA & English \\
    \hline
    \RaggedRight{\begin{arabtext} \smallالاستقلال المحتمل لمونتينيغرو \textbf{يحدث شرخا} بين سكانها \end{arabtext}} & The potential independence of Montenegro is \textbf{causing a rift} among its population \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small  و إذا كان هناك من يتصور إمكانية تحقيق هدنة بدون أي أفق سياسي، فإنه \textbf{يجري وراء سراب}. \end{arabtext}} & And if someone imagines the possibility of achieving a truce without any political horizon, then he is \textbf{running behind a mirage}. \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small  لقاء مونتوبان: عودة سوتومايور \textbf{تتكلل بالنجاح}. \end{arabtext}} & Montauban meeting: The returning of Sotomayor is \textbf{crowned with success}. \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small استعد \textbf{لدخول دائرة الضوء} إذا كنت ترغب في تنمية طموحاتك \end{arabtext}} & Get ready to \textbf{step into the light circle} if you want to grow your ambitions. \\ 
    \hline
    \end{tabular}
    \caption{Examples from the Multi Word Expressions (MWEs) dataset and their English translations.}
    \label{tab:mwe_examples}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proverbs Translation} 
We collected \todo{Add total number} of proverbs in MSA and DA along with (1) their literal English translations and (2) their equivalent English proverbs.  
100 proverbs in MSA were selected from websites teaching Arabic as a foreign language. 150 Egyptian proverbs were additionally collected from websites teaching Egyptian Arabic to non-natives along with their meanings in English. Lastly, 100 Moroccan proverb were gathered from \cite{todo} before translating them to English.
\subsubsection{Multi-Word Expressions Translation}
We collected 100 sentences of verbal MWEs in Modern Standard Arabic from the PARSEME dataset \cite{mohamed2022annotating}.
\todo{Define MWEs (+ diff w/ collocs) + selection criteria if any + we translated them professionally}
Table \ref{tab:mwe_examples} shows examples of said MWEs with their English translations.

\begin{table*}[t]
    \centering
    \begin{tabular}{|p{0.5\linewidth}|p{0.5\linewidth}|}
    \hline
    MSA & English \\
    \hline
    \RaggedRight{\begin{arabtext} \smallالاستقلال المحتمل لمونتينيغرو \textbf{يحدث شرخا} بين سكانها \end{arabtext}} & The potential independence of Montenegro is \textbf{causing a rift} among its population \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small  و إذا كان هناك من يتصور إمكانية تحقيق هدنة بدون أي أفق سياسي، فإنه \textbf{يجري وراء سراب}. \end{arabtext}} & And if someone imagines the possibility of achieving a truce without any political horizon, then he is \textbf{running behind a mirage}. \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small  لقاء مونتوبان: عودة سوتومايور \textbf{تتكلل بالنجاح}. \end{arabtext}} & Montauban meeting: The returning of Sotomayor is \textbf{crowned with success}. \\ 
    \hline
    \RaggedRight{\begin{arabtext} \small استعد \textbf{لدخول دائرة الضوء} إذا كنت ترغب في تنمية طموحاتك \end{arabtext}} & Get ready to \textbf{step into the light circle} if you want to grow your ambitions. \\ 
    \hline
    \end{tabular}
    \caption{Examples from the Multi Word Expressions (MWEs) dataset and their English translations.}
    \label{tab:mwe_examples}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Proverbs Translation} 
We collected \todo{Add total number} of proverbs in MSA and DA along with (1) their literal English translations and (2) their equivalent English proverbs.  
100 proverbs in MSA were selected from websites teaching Arabic as a foreign language. 150 Egyptian proverbs were additionally collected from websites teaching Egyptian Arabic to non-natives along with their meanings in English. Lastly, 100 Moroccan proverb were gathered from \cite{todo} before translating them to English.
\todo{Should we make all the numbers the same?}
Examples of these proverbs are provided in Table \ref{tab:proverb_examples}.

\begin{table}[]
    \centering
    \begin{tabular}{|c|p{0.7\linewidth}|}
    \hline
    Variety & Examples \\
    \hline
    \multirow{2}{*}{MSA} & \RaggedRight{\begin{arabtext} \small تجري الرياح بما لا تشتهي السّفن.\end{arabtext}}\\ 
    \cline{2-2}
    & \RaggedRight{\begin{arabtext}مصائب قوم عند قوم فوائد.\end{arabtext}}\\
    \hline
    \multirow{2}{*}{EGY} & \RaggedRight{\begin{arabtext} \small سَبْع ولّا ضَبْع؟ \end{arabtext}}\\ 
    \cline{2-2}
    & \RaggedRight{\begin{arabtext}كلّه عند العرب صابون.\end{arabtext}}\\
    \hline
    \multirow{2}{*}{MOR} & \RaggedRight{\begin{arabtext} \small كون كان الخوخ يداوي كون داوا راسو\end{arabtext}}\\ 
    \cline{2-2}
    & \RaggedRight{\begin{arabtext} \small طلع تاكل الكرموس هبط شكون قالها ليك\end{arabtext}}\\
    \hline
    \end{tabular}
    \caption{Examples from each of the Arabic varieties in the proverbs datasets. MSA: Modern Standard Arabic. EGY: Egyptian Dialect. MOR: Moroccan Dialect.}
    \label{tab:proverb_examples}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Syntactic Ambiguity Translation}\label{subsec:synAmbData}
Among the linguistic features that we test ChatGPT on is its ability to translate syntactically ambiguous sentences in Arabic. 
Syntactic ambiguity is a pervasive occurrence in natural language, generally arising when a word or a sequence of words exhibits more than one possible interpretation. This ambiguity is primarily of two types: \textbf{syntactic} and \textbf{lexical}. Syntactic ambiguity manifests when a phrase or sentence is susceptible to multiple syntactic interpretations. On the other hand, lexical ambiguity arises when a single word carries more than one meaning.
The ambiguity inherent to the Arabic language is principally a result of parsing. Other sources of ambiguity can stem from factors such as sentence length, the complexity of the Arabic syntax, the omission of diacritical marks in written Arabic ("Tashkiil"), and the elliptical use of personal pronouns (\textAR{الضمير المستتر}). In this paper, we studied various ambiguous cases from the Arabic language, which include the use of:

\begin{itemize}
    \item Abbreviated nouns
    \item Suffixed personal pronouns
    \item Coordination
    \item Comparison
    \item Adverbs
    \item Prepositional phrase attachment
    \item Prenominal references
\end{itemize}

% 1. the use of abbreviated nouns, 
% 2. the use of the suffixed personal pronoun,
% 3.  the use of coordination, 
% 4. the use of comparison, 
% 5. the use of adverbs, 
% 6. prepositional phrase attachment
% 7.  prenominal reference.

Several forms contribute to the structural ambiguity in Arabic. A clear-cut example of this phenomenon is the use of abbreviated nouns. Consider the sentence: \textAR{ضرب موسى عيسى} (Moses hit Iessa). The sentence's ambiguity lies in using abbreviated nouns "Moses" and "Iessa," which lack case markings. Consequently, whether "Moses" is the sentence’s subject or object becomes unclear. It can be interpreted as either "Moses" being the subject or "Iessa."
Another case of syntactic ambiguity is the use of suffixed personal pronouns. For instance: \textAR{اخبر أحمد علياً أنه مخطى} (Ahmed told Ali that he was wrong). The ambiguity here arises due to the suffixed personal pronoun (hu) in (\textAR{أنه}), which could modify either the subject (Ahmed) or the object (Ali). Hence, the sentence could be interpreted as either "Ahmed told Ali [that Ahmed was wrong]" or "Ahmed told Ali [that Ali was wrong]."

We accumulated a collection of 35 instances of such MSA sentences derived from a range of theses exploring this particular feature of Arabic \cite{بن2021الالتباس}. 
Table \ref{tab:synAmb_examples} showcases some examples of ambiguous sentences with the two meanings they can take.
 
% One of the linguistic features we are testing is ChatGPT's ability to translate syntactic ambiguous sentences in Arabic. We collected 40 MSA ambiguous sentences from different theses tackling this feature in the Arabic language. 

\begin{table*}[t]
    \centering
    \begin{tabular}{|m{0.26\linewidth}|m{0.26\linewidth}|m{0.26\linewidth}|}
    \hline
    \Centering{Example} & \Centering{Meaning 1} & \Centering{Meaning 2} \\
    \hline
    \RaggedRight{\begin{arabtext} \small جاء الآباء والأبناء المتميزون \end{arabtext}} & The distinguished fathers and sons came & The fathers and the distinguished sons came\\ 
    \hline
    \RaggedRight{\begin{arabtext} \small قال أحمد في المسجد يصلي الناس. \end{arabtext}} & Ahmed said that people pray in the mosque & Ahmed said in the mosque that people pray\\ 
    \hline
    \RaggedRight{\begin{arabtext} \small انقاذ أهرامات مصر القديمة \end{arabtext}} & The rescue of the ancient pyramids of Egypt & The rescue of the pyramids of ancient Egypt\\ 
    \hline
    \end{tabular}
    \caption{Examples from the syntactic ambiguity dataset with their two possible English translations.}
    \label{tab:synAmb_examples}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Lexical Relations Datasets}\label{subsec:lexRelData}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Collocations}\label{subsec:collocData}
%\todo{Add description, what are collocations + how many collected, source etc.}
Collocation is a distinctive linguistic feature inherent to any language, characterized by the occurrence of specific words together. It exhibits an unpredictable tendency to select one word over another, which can be attributed to its arbitrary nature. "collocations" denotes the simultaneous appearance of two or more words. Collocations hold significant importance within a language, primarily contributing to the coherence of its overall structure. Ghazala \cite{ghazala1993translation}defines collocation as “words which are usually found next to each other or are ‘co-located’ with one another.”
We compiled a set of 50 Arabic collocations from Al-Hafez dictionary \cite{hafiz2004hafiz} Dictionary. Our selection criteria primarily focused on words that exhibited a wide range of collocates, ranging from a minimum of two words to a maximum of ten words. This approach aimed to provide deeper insights into CGPT's ability to form collocations accurately. The study examined two types of collocations: grammatical and lexical collocations. These encompassed combinations such as nouns/adjectives, adjectives/prepositions, and nouns in the genitive construct, among others.
Additionally, we investigated another set of 50 collocations that were restricted in nature, specifically onomatopoeic collocations and collective words.
Table \ref{tab:colloc_examples} presents examples of the collected collocations.

\begin{table}[]
    \centering
    \begin{tabular}{|m{0.26\linewidth}|m{0.26\linewidth}|m{0.26\linewidth}|}
    \hline
    \Centering{MSA Collocation} & \Centering{MSA Co-Occurence} & \Centering{English} \\
    \hline
    \multirow{4}{\linewidth}{\Centering{\begin{arabtext} \small ثنائي \end{arabtext}}} & \Centering{\begin{arabtext} \small البعد \end{arabtext}} & \Centering{Two-dimensional}\\ 
    \cline{2-3}
    & \Centering{\begin{arabtext} \small التكافؤ \end{arabtext}} & \Centering{Bivalent}\\
    \cline{2-3}
    & \Centering{\begin{arabtext} \small الحد \end{arabtext}} & \Centering{Binomial}\\
    \cline{2-3}
    & \Centering{\begin{arabtext} \small الخلية \end{arabtext}} & \Centering{Bicellular}\\
    \hline
    \multirow{4}{\linewidth}{\Centering{\begin{arabtext} \small رقيق \end{arabtext}}} & \Centering{\begin{arabtext} \small الحال \end{arabtext}} & \Centering{Poor}\\ 
    \cline{2-3}
    & \Centering{\begin{arabtext} \small الشعور \end{arabtext}} & \Centering{Sensitive}\\
    \cline{2-3}
    & \Centering{\begin{arabtext} \small القلب \end{arabtext}} & \Centering{Soft-hearted}\\
    \hline
    \end{tabular}
    \caption{Examples from the collocations dataset with their English translations.}
    \label{tab:colloc_examples}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Synonyms and Antonyms Datasets}\label{subsec:provData}
We curate a collection of 50 Egyptian words from the Dialex dataset \cite{abdul2020dialex} and 50 Moroccan words from the DODa dataset \cite{outchakoucht2021moroccan}, focusing on the following criteria: 
\begin{itemize}
    \item We exclusively choose words that possess antonyms, thus excluding words such as "cake".
    \item We only select words that have no origin in other languages, thereby avoiding code-switching instances like the Moroccan word for "ticket" (\textAR{تيكي}).
    \item We prioritize words that differ in pronunciation from their corresponding MSA translations, eliminating words like the Egyptian term for "a lot" (\textAR{كتير}).\todo{Still need to discuss this}
\end{itemize}
Examples from the synonyms and antonyms dataset can be found in Table \ref{tab:synant_examples}

\begin{table}[]
    \centering
    \begin{tabular}{|c|m{0.20\linewidth}|m{0.20\linewidth}|m{0.20\linewidth}|}
    \hline
    \Centering{Variety} & \Centering{Word} & \Centering{Synonyms} & \Centering{Antonyms} \\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MSA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\Centering{MSA}} & \multirow{3}{\linewidth}{ \Centering{\begin{arabtext} \small مرح \end{arabtext} Happiness Fun}} & \Centering{\begin{arabtext} \small سعادة  \end{arabtext}} & \Centering{\begin{arabtext} \small حزن   \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small بهجة \end{arabtext}} & \Centering{\begin{arabtext} \small كآبة \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small فرح  \end{arabtext}} & \Centering{\begin{arabtext} \small ضجر \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small لطيف \end{arabtext} Kind}} & \Centering{\begin{arabtext} \small حسن \end{arabtext}} & \Centering{\begin{arabtext} \small قاسي \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small رقيق \end{arabtext}} & \Centering{\begin{arabtext} \small سيء \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small طيب \end{arabtext}} & \Centering{\begin{arabtext} \small بغيض \end{arabtext}}\\ 
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EGY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{5}{*}{\Centering{EGY}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small كويس \end{arabtext} Good}} & \Centering{\begin{arabtext} \small حلو  \end{arabtext}} & \Centering{\begin{arabtext} \small سيء   \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small زي الفل \end{arabtext}} & \Centering{\begin{arabtext} \small رديء \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small تمام   \end{arabtext}} & \Centering{\begin{arabtext} \small مش قد كده \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{2}{\linewidth}{\Centering{\begin{arabtext} \small كحيان \end{arabtext} Poor}} & \Centering{\begin{arabtext} \small مسكين \end{arabtext}} & \Centering{\begin{arabtext} \small مريًش \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small غلبان \end{arabtext}} & \Centering{\begin{arabtext} \small غني \end{arabtext}}\\ 
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MOR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{5}{*}{\Centering{MOR}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small مكلخ \end{arabtext} Stupid}} & \Centering{\begin{arabtext} \small عبيط \end{arabtext}} & \Centering{\begin{arabtext} \small ذكي \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small بليد \end{arabtext}} & \Centering{\begin{arabtext} \small مطور \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small مطنگ  \end{arabtext}} & \Centering{\begin{arabtext} \small معلم \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{2}{\linewidth}{\Centering{\begin{arabtext} \small معصب \end{arabtext} Angry}} & \Centering{\begin{arabtext} \small غضبان \end{arabtext}} & \Centering{\begin{arabtext} \small فرحان \end{arabtext}}\\ 
    \cline{3-4}
    & & \Centering{\begin{arabtext} \small كاعي \end{arabtext}} & \Centering{\begin{arabtext} \small مرتاح \end{arabtext}}\\ 
    \hline
    \end{tabular}
    \caption{Examples from the synonyms and antonyms dataset. MSA: Modern Standard Arabic. EGY: Egyptian Dialect. MOR: Moroccan Dialect.}
    \label{tab:synant_examples}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Hypernyms and Hyponyms}
\todo{Add description, what are hyps + how many collected, source etc.}

Example words and they respective hypernyms and hyponyms are listed in Table \ref{tab:hyp_examples}.


\begin{table}[]
    \centering
    \begin{tabular}{|c|m{0.20\linewidth}|m{0.20\linewidth}|m{0.20\linewidth}|}
    \hline
    \Centering{Variety} & \Centering{Word} & \Centering{Hypernym} & \Centering{Hyponyms} \\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MSA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\Centering{MSA}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small عمل \end{arabtext} Work\\Job}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small مهنة  \end{arabtext}}} & \Centering{\begin{arabtext} \small مهندس   \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small طبيب \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small معلم  \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small دراجة \end{arabtext} Bike}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small وسيلة نقل \end{arabtext}}} & \Centering{\begin{arabtext} \small دراجة جبلية \end{arabtext}}\\ 
    \cline{4-4}
    % & & & \Centering{\begin{arabtext} \small دراجة هوائية \end{arabtext}}\\ 
    % \cline{4-4}
    & & & \Centering{\begin{arabtext} \small دراجة بي إم إكس \end{arabtext}}\\ 
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EGY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\Centering{EGY}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small حنفية \end{arabtext} Faucet}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small أدوات الصرف الصحي  \end{arabtext}}} & \Centering{\begin{arabtext} \small حنفية المطبخ   \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small حنفية الدش \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small حنفية الحديقة  \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small شبشب \end{arabtext} Flip-flop}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small جزمة \end{arabtext}}} & \Centering{\begin{arabtext} 
    \small شبشب نسائي \end{arabtext}}\\ 
    \cline{4-4}
    % & & & \Centering{\begin{arabtext} \small شبشب حمام  \end{arabtext}}\\ 
    % \cline{4-4}
    & & & \Centering{\begin{arabtext} \small شبشب شاطئ \end{arabtext}}\\ 
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MOR %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \multirow{6}{*}{\Centering{MOR}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small خامية \end{arabtext} Curtain}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small أتات \end{arabtext}}} & \Centering{\begin{arabtext} \small خامية ديال الشرجم   \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small خامية ديال الحمام \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small خامية ديال المسرح  \end{arabtext}}\\ 
    \cline{2-4}
    & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small مكينة \end{arabtext} Machine}} & \multirow{3}{\linewidth}{\Centering{\begin{arabtext} \small أداة \end{arabtext}}} & \Centering{\begin{arabtext} \small مكينة ديال الخياطة \end{arabtext}}\\ 
    \cline{4-4}
    & & & \Centering{\begin{arabtext} \small مكينة ديال الحسانة \end{arabtext}}\\ 
    % \cline{4-4}
    % & & & \Centering{\begin{arabtext} \small مكينة ديال القهوة \end{arabtext}}\\ 
    \hline
    \end{tabular}
    \caption{Examples from the hypernyms and hyponyms dataset. MSA: Modern Standard Arabic. EGY: Egyptian Dialect. MOR: Moroccan Dialect.}
    \label{tab:hyp_examples}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Prompts Design} 
% ChatGPT is mainly a large language model that needs well-designed prompts to trigger its ultimate performance because such models are sensitive to the prompts provided. Therefore, Prompts play a key role in unleashing ChatGPT's linguistic abilities. Since we are testing different linguistic features of ChatGPT, we designed various prompts that meet our targets for translation and  linguistic abilities in Arabic. 





==> Sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

==> Sections/error-analysis-CGPT.tex <==

%\subsection{Error Analysis of ChatGPT and GPT-4}
%\textcolor{purple}{\textbf{(K)}

\noindent{\textbf{Error Analysis.}} To further investigate translation quality, we carry out an analysis of the 0-shot ChatGPT and GPT-4 translations of $50$ sentences from the Moroccan and Egyptian dialect sets. We find that that the two systems can struggle when translating \textit{idiomatic expressions} ingrained within the dialects, cases of \textit{code-switching}, \textit{named entities}, \textit{tense},  \textit{homonymy}, and \textit{polysemy}. We provide details of our error analysis in Appendix~\ref{appendix-cgpt-error-analysis}, along with illustrating examples (Table~\ref{tab:cgpt-error-analysis}).


% We then identify reoccurring error categories that span semantic, syntactic, grammatical and lexical dimensions. Namely:
% \\
% \textbf{Idiomatic Errors:} The literal translation of multi-word expressions (MWEs), proverbs, and other region-specific language.
% \\
% \textbf{Code-Switching Errors:} Including both undetected code-switched words as well as dialectal words inaccurately treated as code-switched elements.
% \\
% \textbf{Named Entity Errors:} The literal translation of proper nouns or their substitution with different ones.
% \\
% \textbf{Tense Errors:} Alterations of verb tenses.
% \\
% \textbf{Addition/Omission Errors:} The presence of words in the target that don't appear in the source, as well as the leaving out of source words in the translation.
% \\
% \textbf{Polysemy Errors:} A source word with two or more related meanings being translated into the wrong meaning.
% \\
% \textbf{Homonymy Errors:} Translating from the homonym of the source word instead of the intended word itself.
% \\
% Examples of these errors are presented in Table \ref{tab:cgpt-error-analysis} in Appendix \ref{appendix-cgpt-error-analysis}.
% 



==> Sections/methodology_prev.tex <==
\section{Methodology}\label{sec:methodology}

\subsection{Prompts Design} 
% One of our primary aims is to contrast the translations produced by ChatGPT 3.5 and 4. 
Various studies have examined ChatGPT's proficiency as a translation instrument, with many emphasizing the crucial role of prompts in optimizing translation outcomes. 
% This report scrutinizes ChatGPT's translation capabilities across various Arabic varieties, including Classical Arabic, Modern Standard Arabic, and dialectal Arabic (Egyptian and Moroccan). 
We employed previously designed prompts while also modifying some of them to meet our translation objectives effectively, particularly regarding dialectal Arabic. We chose prompts across diverse domains, which aid ChatGPT in accurately identifying and translating the texts. Using prompts, including instructions to translate from the source to the target language, has proven to be a successful strategy in obtaining high-quality translations from ChatGPT.

 \begin{itemize}
      \item \textbf{Arabic Varieties Translation:}
 The initial assessment in our evaluation process involves examining the translation abilities of ChatGPT. Consequently, we used prompts that encompass the domain related to the specific variety under scrutiny to achieve optimal performance. 
 % Using a zero-shot, w
 We queried ChatGPT with the prompt, "\textit{Translate the following [Arabic Variety] sentence into English: [Sentence]}" employing both zero and five-shot approaches.
 % We employed both zero-shot and five-shot prompts to evaluate Dialectal Arabic (DA) to ensure enhanced performance.
       \item \textbf{Paraphrasing:}
 % In order to evaluate CGPT's linguistic competencies, we experimented with several prompts targeting the tasks we tested.
 We assessed its capability to paraphrase Arabic sentences across CA, MSA, and DA (Egyptian and Moroccan variants). For CA and MSA, we utilized a prompt that requested ChatGPT to provide five alternative paraphrases in Arabic for a given CA sentence. 
 % It was essential to specify the particular variety of Arabic we were examining. 
 A more effective prompt for Dialectal Arabic was: "\textit{I will give you a sentence in Egyptian Arabic dialect, and I want you to paraphrase it into five different sentences in Egyptian Arabic dialect: [Sentence]}” Compared to other prompts, this one demonstrated better performance in paraphrasing in the Dialectal Arabic.
       \item \textbf{Proverbs Translation:}
 In our endeavor to analyze the translation performance for proverbs, we experimented with various prompts. Initially, we tasked ChatGPT with translating an MSA proverb into its English equivalent. Although most translations were literal, this prompt showed satisfactory results with certain well-known proverbs. Consequently, we explored an alternative prompt that demonstrated effectiveness with both MSA and Dialectal Arabic. This prompt was: "I will give you a proverb in Egyptian, and I want you to give me the English proverb that is used in the same situation but isn't a direct translation: [Proverb]". It was observed that ChatGPT could interpret the proverbs we were translating without being explicitly asked to generate such explanations.
 \item \textbf{Synonyms and Antonyms:}
 In relation to ChatGPT's lexical capacity for understanding and translating synonyms and antonyms in both MSA and DA, we designed prompts tailored to elicit the targeted outputs. For MSA, the initial prompt was: "I will give you a word in MSA, and I want you to give me some synonyms and antonyms of that word in MSA. The word is: [word]." When the response fell short of expectations, we employed an alternative prompt designed to guide CGPT toward the correct word. This prompt was: "The word actually means "[word in English]." Can you give me synonyms and antonyms for that word in the MSA?". These two prompts were applied to Dialectal Arabic for both Egyptian and Moroccan varieties and showed satisfactory results with certain words, mainly when using CGPT 4. The prompts used for Dialectal Arabic were: "I will give you a word in Moroccan Arabic, and I want you to give me some synonyms and antonyms of that word in Moroccan Arabic. The word is: [word].” The other prompt is: "The word actually means "[word in English].” Can you give me synonyms and antonyms for that word in the Moroccan dialect?".
 \item \textbf{Hypernym and Hyponyms:}
We used three different prompts to evaluate hypernyms and hyponyms in MSA and Dialectal Arabic using CGPT. The first two were primarily employed with CGPT 3.5, as it may require assistance in understanding the dialectal words for which we sought responses. Initially, we asked CGPT about the English meaning of the dialectal word. If CGPT's answers were accurate, we would then present the second prompt, asking for the hypernyms and hyponyms of the word in, for example, Egyptian Arabic. These prompts were written as follows: "What does this Egyptian Arabic dialect word mean: [word]." "What are the hypernym and hyponyms of the Egyptian Arabic dialect word "[word].”
When testing Dialectal Arabic words with CGPT4, we found that a more direct prompt revealed better results. The prompt was: "I will give you an Egyptian Arabic dialect word, and I want you to give me its hypernym and hyponyms in the Egyptian Arabic dialect: "[word]."  We employed the same prompt when generating hypernyms and hyponyms in MSA.

\item \textbf{Syntactic Ambiguous Sentences:}
In our efforts to generate translations for syntactically ambiguous sentences, we utilized numerous prompts with ChatGPT. Initially, we prompted ChatGPT to translate the sentence without explicitly referencing the ambiguity using the following prompt: “Please provide a list of the English translation for these Arabic sentences,” and we expect CGPT to detect the ambiguity and give the two different meanings that the sentence could convey. Then we use the prompt “[This sentence is syntactically ambiguous. Please provide the two different possible translations for the Arabic sentence:”] to assess the ability of CGPT to find the different meanings when it does not detect ambiguity.
\end{itemize}
 


 

==> Tables/CGPT-error-analysis.tex <==
\begin{landscape}

\begin{table}[]
    \centering
    \begin{tabular}{llrp{0.4\textwidth}p{0.4\textwidth}}
    \toprule
        \textbf{Category} & \textbf{Dia} & \multicolumn{1}{c}{\centering \textbf{Source}} & \multicolumn{1}{c}{\textbf{Reference}} & \multicolumn{1}{c}{\textbf{Example}}  
        % & \textbf{System} 
        \\
    \midrule
        \multirow{2}{*}{Idiomatic} & \small EGY & \small \< بقولك خالد \textbf{فص ملح و داب}> & \small I am telling you that Khalid has \textcolor{red}{vanished}. & \cellcolor{Plum!15} \small I'm telling you Khalid is the \textcolor{red}{salt of the earth}. 
        % & \small GPT-4
        \\
        
        & \small MOR & \small \<\textbf{ها العار} لا كنتي عارف شي حاجة لما قلها ليا.> & \small \textcolor{red}{I beg you} to tell me if you know something. & \cellcolor{LimeGreen!15}\small \textcolor{red}{This is shameful} if you knew something and didn't tell me.  
        % & \small ChatGPT
        \\
    \midrule     
    
        Code-Switching & \small MOR & \small \<هاد الرجل را جبتو من \textbf{البيرو} ديال الجماعة.> & \small I brought this guy from the \textcolor{red}{office} of the Commune. & \cellcolor{Plum!15} \small I brought this man from the community's \textcolor{red}{well}.
        % & \small GPT-4
        \\
    \midrule
        
        \multirow{2}{*}{Named Entity} & \small EGY & \small \<أكتر من كده هيبقى جيش يا \textbf{رفقي}> & \small More than this, it will be an army \textcolor{red}{Refky} & \cellcolor{LimeGreen!15} \small More than that, it will be an army, \textcolor{red}{my friend}. 
        % & \small ChatGPT 
        \\

        
        & \small MOR & \small \<لاش غتحشمي آ \textbf{عواطف}؟> & \small Why would you be shy \textcolor{red}{Awatef}? & \cellcolor{LimeGreen!15} 
        \small Why are you ashamed \textcolor{red}{of your feelings}? 
        % & \small ChatGPT
        \\
    \midrule
        
        Tense & \small MOR & \small \<ووحدة \textbf{غتاخد} الوقت.> & \small And one \textcolor{red}{will take} time. & \cellcolor{LimeGreen!15} \small And one \textcolor{red}{takes} time.\\

    \midrule
        
        % \multirow{2}{*}{Wrong Subject} & \small EGY \<> \\
        % & \\
        
        % \multirow{2}{*}{Word Order} & \\
        
        % & \\
        
        \multirow{2}{*}{Addition} & \small EGY & \small \< كل المحاضرات اللي كانت نقصاكي معاكي>
        % \\ \small \<كانت نقصاكي معاكي> }
        & \small You have all the lectures you were missing. & \cellcolor{LimeGreen!15} \small All the lectures that you missed, \textcolor{red}{we have covered them with you}.
        % & ChatGPT 
        \\ 
        
         & \small MOR & \small\<داك النهار تلاقيت مع مي فريحة. > &  \small That day I met Mom Fariha. & \cellcolor{LimeGreen!15}  \small That day, I met with \textcolor{red}{my friend} Me Farihah. 
         % & ChatGPT
         \\
    \midrule
        Omission & \small EGY & \small \<طب اقعد أعمل كوبيتين شاي> & \small Okay \textcolor{red}{sit down}, and I'll make two cups of tea. & \cellcolor{LimeGreen!15} \small Okay, let me make two cups of tea.\\
    \midrule
        Polysemy & \small EGY & \small \<أنا عايزك تجنن العيال دي> & \small I want you to drive these guys \textcolor{red}{crazy}. & \cellcolor{LimeGreen!15} \small I want you to \textcolor{red}{amaze} these kids. \\
    \midrule  
        Homonymy & \small MOR & \small \<واش أنا بنت ليك ناقصة مشاكل؟> & \small Do I \textcolor{red}{seem} like I don't have enough problems? & \cellcolor{Plum!15} \small Do you think I, \textcolor{red}{your daughter}, am short of problems?\\
         
    \bottomrule
    \end{tabular}
    \caption{Some translation error categories met with \colorbox{LimeGreen!15}{ChatGPT} and \colorbox{Plum!15}{GPT-4} under the 0-shot setting.}
    \label{tab:cgpt-error-analysis}
\end{table}

\end{landscape}

==> Tables/MT_Examples-old.tex <==

% \begin{landscape}
\begin{table*}[h]
    \centering
    \footnotesize 
    \renewcommand{\arraystretch}{0.9}   %to squeeze table content low value means squeeze more
    \resizebox{1.\linewidth}{!}{% reduce the text size, lower means smaller text size
    \begin{tabular}{c p{0.4 \linewidth} p{0.4\linewidth}}
    % \begin{tabular}{|c|p{0.5 \linewidth}|p{0.5 \linewidth}|}
    \toprule
    \textbf{Variety} & \Centering{\textbf{Arabic}} & \textbf{~~~~~~~~~~~~~ English}\\
    \midrule
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%     CA & \RaggedRight{

% \begin{arabtext} \small وَاعْلَمْ أَنَّ لِكُلِّ مَطْلُوبٍ بَاعِثًا. وَالْبَاعِثُ عَلَى الْمَطْلُوبِ شَيْئَانِ رَغْبَةٌ أَوْ رَهْبَةٌ، فَلْيَكُنْ طَالِبُ الْعِلْمِ رَاغِبًا رَاهِبًا.  \end{arabtext}    
%     } & And know that everything you want should have a motivation. And what motivates a person to get what he wants is either a desire or awe, so the seeker of knowledge should be both desirous and anchorite.\\\\
    % \multirow{2}{*}{CA} & \RaggedRight{\begin{arabtext} \small وكانت بنو مليح من خزاعة وهم رهط طلحة الطلحات يعبدون الجن\end{arabtext}} & Banū Malī\d{h}, Raht Tal\d{h}aht El-Tal\d{h}at, tribe which descended from Khuza'ah tribe, used to worship Jinn.\\ 
    % \cline{2-3}
    % &  \RaggedRight{\begin{arabtext} \small فغاية الناس وحاجاتهم صلاح المعاش والمعاد، والسبيل إلى دركها العقل الصحيح.\end{arabtext}} & The ultimate goal or need that people seek is creating a better life and afterlife; and common sense is the only means to reach them.\\
    % \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \rowcolor{blue!5} MSA & \RaggedRight{\begin{arabtext} \small اكتسح مانشستر سيتي مضيفه ساوثهامبتون 4-1 اليوم السبت ضمن منافسات الجولة 30 من الدوري الإنجليزي لكرة القدم. \end{arabtext}} & On this Saturday, Manchester City swept Southampton 4-1, in the 30th round of the English Premier League.\\ 
    % \cdashline{1-3}\\
    % % \multirow{2}{*}{MSA} & \RaggedRight{\begin{arabtext} \small اكتسح مانشستر سيتي مضيفه ساوثهامبتون 4-1 اليوم السبت ضمن منافسات الجولة 30 من الدوري الإنجليزي لكرة القدم. \end{arabtext}} & On this Saturday, Manchester City swept Southampton 4-1, in the 30th round of the English Premier League.\\ 
    % % \cline{2-3}
    % % & \RaggedRight{\begin{arabtext} \small شهدت أسهم البنوك حول العالم تراجعا حادا وسط مخاوف من تعرّض بنوك أخرى لمشكلات مشابهة، ومن اندفاع المستثمرين إلى سحب أموالهم.\end{arabtext}} & Bank stocks around the world witnessed a sharp decline amid fears that other banks would be exposed to similar problems, and that investors would rush to withdraw their money.\\
    % % \toprule
    % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %     ALG  & \RaggedRight{\begin{arabtext} \small القصر نعرفو كي جيبي كاين واحد الدخلة تدينا ديراكت للحبس \end{arabtext}} & I know the castle like the back of my hand. There's an entrance that will take us directly to the prison. \\ 
    % \multirow{2}{*}{ALG} & \RaggedRight{\begin{arabtext} \small   \end{arabtext}} & \\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small \end{arabtext}} & \\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \rowcolor{blue!5} EGY & \RaggedRight{\begin{arabtext} \small ماحنا لو فضلنا مدارين و مستخبين هنموت من الخوف. \end{arabtext}} & And if we keep hiding, we’re going to die out of fear.\\ 
    % \multirow{2}{*}{EGY} & \RaggedRight{\begin{arabtext} \small ماحنا لو فضلنا مدارين و مستخبين هنموت من الخوف. \end{arabtext}} & And if we keep hiding, we’re going to die out of fear.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small طب اقعد أعمل كوبيتين شاي من بتوع زمان و نقعد ندردش براحتنا. \end{arabtext}} & Just go make some tea, tea of the old days, so we can chill and talk\\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    JOR & \RaggedRight{\begin{arabtext} \small   أنا مش مستخف فيه و لا يمكن استخف فيه مهما كان بضل ابوي\end{arabtext}} & I do not and cannot underestimate him; he is still my father, no matter what.\\ 
    % \multirow{2}{*}{JOR} & \RaggedRight{\begin{arabtext} \small   أنا مش مستخف فيه و لا يمكن استخف فيه مهما كان بضل ابوي\end{arabtext}} & I do not and cannot underestimate him; he is still my father, no matter what.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small لا فترة قصيرة ولا اشي، أنا صارلي عايشه بينهم اكثرمن شهرين وأظن هالفترة كافية مشان اعرف عنهم كل اشي\end{arabtext}} & It is not a short time. Having lived with them for over two months, I feel that I have sufficient time to become familiar with every aspect of their lives.\\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \rowcolor{blue!5} MAU & \RaggedRight{\begin{arabtext} \small   شوف آن شي كامل ادخلتو ماتيت انركيلي فيه خالك اللا القدام.\end{arabtext}} & Look, whenever I'm in, I never take a step back; I only go forward.\\ 
    % \multirow{2}{*}{MAU} & \RaggedRight{\begin{arabtext} \small   شوف آن شي كامل ادخلتو ماتيت انركيلي فيه خالك اللا القدام.\end{arabtext}} & Look, whenever I'm in, I never take a step back; I only go forward.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني انو بدو يبقى ياران لك ملي ما فايتن علنك ما تيت تقعد هون في البوتيك\end{arabtext}} & For your record, we are aware that you no longer sit with us in the store.\\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % % uncomment this if you want it to be there
    % MOR & \RaggedRight{\begin{arabtext} \small بحالا علمك الله آ سي علي. شفت كلشي. و دابا را كلشي ولا باين و ما بقى ما يتخبى.\end{arabtext}} & It's as if God warned you, Mr. Ali. I saw everything. And now everything became clear and there is nothing to hide anymore\\ 
    % \multirow{2}{*}{MOR} & \RaggedRight{\begin{arabtext} \small بحالا علمك الله آ سي علي. شفت كلشي. و دابا را كلشي ولا باين و ما بقى ما يتخبى.\end{arabtext}} & It's as though God warned you, Mr. Ali. I saw everything. And now everything became clear and there is nothing to hide anymore\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small لا لا، جيت هي نشوف نادية على شي غرض. بغيت غي نسولها على شي حاجة.\end{arabtext}} & No, no. I just came to see Nadia for something. I just want to ask her about something.\\
    % \hline

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % %  uncomment this if you want it to be there
    % \rowcolor{blue!5} PAL & \RaggedRight{\begin{arabtext} \small   يا رب هالاجتماع يخلص بسرعة لأنه عمي أبو العبد اذا بضل يفوتلنا من قصة و يطلعلنا من قصة الكلاسيكو بروح علينا.\end{arabtext}} & God I hope this meeting ends quickly because if uncle Abu al Abed keeps rambling we will miss the Classico.\\ 
    % \multirow{2}{*}{PAL} & \RaggedRight{\begin{arabtext} \small   يا رب هالاجتماع يخلص بسرعة لأنه عمي أبو العبد اذا بضل يفوتلنا من قصة و يطلعلنا من قصة الكلاسيكو بروح علينا.\end{arabtext}} & God I hope this meeting ends quickly because if uncle Abu al Abed keeps rambling we will miss the Classico.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني انو بدو يبقى يا سيدي، معقول شرطة من الداخلية أو سيارة شرطة هيك عابرة سبيل؟.\end{arabtext}} & So who could it be sir, could it be a police from the ministry of the interior or just a police car passing by?\\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % UAE & \RaggedRight{\begin{arabtext} \small لا أنا ما قلت جيه يالياسمينه أنا أقول إن راجح مسوي هالخطة عشان يزخ الحرامي.\end{arabtext}} & No, Yasmina, I did not say that. I'm saying Rajah devised this plan to capture the thief.\\ 
    % \multirow{2}{*}{UAE} & \RaggedRight{\begin{arabtext} \small لا أنا ما قلت جيه يالياسمينه أنا أقول إن راجح مسوي هالخطة عشان يزخ الحرامي.\end{arabtext}} & No, Yasmina, I did not say that. I'm saying Rajah devised this plan to capture the thief.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small ان شاء الله ان شاء الله يا عمي، أنا بس يعني أبغى أخبرك، أقولك شو استوى في الفريج.\end{arabtext}} & God willing, uncle God willing, I just wanted to let you know what happened in the neighborhood.\\
    % \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % \rowcolor{blue!5} YEM & \RaggedRight{\begin{arabtext} \small   ركزت لي نفطة تفتيش، في الباب، بتفتش ذي داخلي و ذي خارجي.\end{arabtext}} & I set up a checkpoint at the door to screen anyone who comes in or out.\\ 
    % \multirow{2}{*}{YEM} & \RaggedRight{\begin{arabtext} \small   ركزت لي نفطة تفتيش، في الباب، بتفتش ذي داخلي و ذي خارجي.\end{arabtext}} & I set up a checkpoint at the door to screen anyone who comes in or out.\\ 
    % \cline{2-3}
    % & \RaggedRight{\begin{arabtext} \small يعني ابي و ابوش هكذا عيجلسوا محبوسين و نحنا نجلس نتفرج.\end{arabtext}} & This means that both my father and your father will be imprisoned, and we will be powerless to intervene.\\
    \hline
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \end{tabular}
    }
    \caption{Example sentences from some of the Arabic varieties in our new translation evaluation dataset. Remaining varieties and their corresponding English references can be found in Appendix table ~\ref{output-samples}. \textcolor{red}{Make size small like Table 2.}}
    \label{tab:variety_examples}
\end{table*}

==> Tables/bard-content-filtering.tex <==
\definecolor{light-blue}{HTML}{D1E5F4}
\definecolor{light-green}{HTML}{BEE3BA}
\definecolor{light-red}{HTML}{FFA8B5}

\begin{table}[]
    \centering
    % \renewcommand*{\arraystretch}{2}
    \begin{tabular}{p{\linewidth}}
    % \begin{tabular}{p{\linewidth} p{\linewidth}
        \toprule
        \makecell[c]{\textbf{\textit{Content Filtering}}} \\
        \midrule

        \begin{tabular}[l]{@{}l@{}} 
            \textbf{Input}: 
            % Translate the following text from\\Moroccan Arabic dialect into English:\\ 
        \end{tabular}  
        \begin{tabular}{r}
            \rowcolor{light-blue!35}\<\small و حتى دوك الرجال لي غنضعافو على ودهم ما عندنا ما>\\
            \rowcolor{light-blue!35}\<\small نديرو بهم.> 
        \end{tabular}\\

        \textbf{Ref:}\\
        \begin{tabular}{l}
            \rowcolor{light-green!35}And even those men for whom we'll become\\
            \rowcolor{light-green!35}thin, we have no use for them.
        \end{tabular}

        \begin{tabular}[l]{@{}l@{}} 
            \textbf{Output}:
        \end{tabular}  
        \begin{tabular}{r}
            \rowcolor{light-red!35}\<\smallمعذرة، لا يمكنني ترجمة هذه الجملة إلى الإنجليزية. إنها >\\
            \rowcolor{light-red!35}\<\small تحتوي على لغة مسيئة.>\\
        \end{tabular} \\
        \bottomrule

        
    \end{tabular}
    \caption{\textcolor{purple}{CHANGE} Examples of errors in Google Bard's ability to follow prompts. For each of the sentences, we use the prompt \textit{Translate the following text from [Variety] Arabic [dialect] into English: <s>}.}
    \label{tab:bard-fails}
\end{table}


==> Tables/content-filtering.tex <==
\begin{table}[t]
\centering
\footnotesize 
 \renewcommand{\arraystretch}{1.4}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{cc}
\toprule
% \multicolumn{2}{c}{\textbf{Content Filtering}}\\ \midrule
\textbf{In} & \begin{tabular}[c]{@{}r@{}}\<\small وحتى دوك الرجال لي غنضعافو على ودهم ما عندنا ما نديرو بهم.>\end{tabular}\\ 


% \multirow{2}{*}{\textbf{Ref}} & \begin{tabular}[c]{@{}r@{}}\<\small أنا مش مستخف فيه و لا يمكن استخف فيه مهما كان بضل ابوي>\end{tabular}\\   
% & \begin{tabular}[c]{@{}l@{}}
% I do not and cannot underestimate him; he is still
% my father, no matter what.\end{tabular}\\ 

\rowcolor{blue!5} \textbf{Ref} & \begin{tabular}[c]{@{}r@{}}And even those men for whom we’ll
become thin, we have no use for them.\end{tabular}\\ 
% And even those men for whom we’ll
% become thin, we have no use for them.


\textbf{Out} & \begin{tabular}[c]{@{}l@{}}
\<\smallمعذرة، لا يمكنني ترجمة هذه الجملة إلِى الإنجليزية. إنها تحتوي على لغة مسيئة.> \end{tabular}\\ 

% \<\smallمعذرة، لا يمكنني ترجمة هذه الجملة إلِى الإنجليزية.>\\
%             % \rowcolor{light-red!35}
%             \<\small  إنها تحتوي على لغة مسيئة.>\\

\bottomrule
\end{tabular}
}
\caption{Example of a \texttt{content\_filtering} error met when translating a sentence from the MOR dialect.}
    \label{tab:content-filtering}
\end{table}

==> Tables/results-tables/bleu-main.tex <==
\input{Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & 0-shot & 1-shot & 3-shot & 5-shot & 0-shot      & 5-shot        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 4.99  & 12.04 & 12.36 & 12.58 & 11.65       & 2.36       & 7.56                  & 7.23                                                                 & 11.28                   & 12.13                & 14.87               \\
% MSA                       & 25.53 & 42.92 & 43.1  & 43.66 & 42.06       & 25.28      & 16.42                 & 41.11                                                                & 46.21                   & 47.1                 & 65.74               \\
% ALG                       & 9.85  & 10.92 & 11.74 & 11.78 & 7.46        & -          & 5.24                  & 4.98                                                                 & 6.68                    & 10.15                & 9.13                \\
% EGY                       & 22.68 & 11.26 & 10.8  & 19.94 & 10.05       & 20.74      & 2.89                  & 6.58                                                                 & 7.49                    & 8.03                 & 8.78                \\
% JOR                       & 24.01 & 24.91 & 26.08 & 24.9  & 22.96       & -          & 10.14                 & 12.86                                                                & 20.66                   & 20.75                & 29.3                \\
% MAUR                      & 7.15  & 7.32  & 7.78  & 7.49  & 7.75        & -          & 2.95                  & 2.75                                                                 & 6                       & 6.09                 & 6.38                \\
% MOR                       & 15.26 & 27.16 & 27.86 & 13.6  & 32.74       & 18.9       & 12.69                 & 10.46                                                                & 12.68                   & 14.27                & 17.02               \\
% PAL                       & 26.86 & 26.85 & 29.3  & 29.18 & 29.42       & 12.11      & 11.80                 & 14.47                                                                & 20.41                   & 24.31                & 23.55               \\
% UAE                       & 23.17 & 23.53 & 23.57 & 24.93 & 21.22       & 11.78      & 9.46                  & 10.93                                                                & 16.27                   & 18.71                & 19.16               \\
% YEM                       & 12.27 & 13.33 & 14.45 & 14.49 & 12.27       & -          & 4.93                  & 8.84                                                                 & 12.95                   & 12.7                 & 11.86               \\
% \midrule
% \textbf{Average}          & 17.18 & 20.02 & 20.70 & 20.26 & 19.76       & 15.20      & 8.41                  & 12.02                                                                & 16.06                   & 17.42 & 20.58  \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{blue-main}
% BLEU Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline with source dialect as MSA.  \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}

% % 2nd table with all bard drafts
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.4}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lcccc|cH|cccc|ccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                        & 4.99   & 12.04  & 12.36  & 12.58  & 11.65       & 2.36        & 12.25 & 10.37	& 12.36	& 11.66  & 7.23                                                                 & -                                                                          & 11.28                   & 12.13                & 14.87               \\
MSA                       & 25.53  & 42.92  & 43.1   & 43.66  & 42.06       & 25.28       & 36.78	& 32.78	& 35.46	& 35.01 & 41.11                                                                & -                                                                          & 46.21                   & 47.1                 & 65.74               \\
ALG                       & 9.85   & 10.92  & 11.74  & 11.78  & 7.46        & -           & 9.16 & 7.49 & 7.59 & 8.08  & 4.98                                                                 & -                                                                          & 6.68                    & 10.15                & 9.13                \\
EGY                       & 22.68  & 11.26  & 10.8   & 19.94  & 10.05       & 20.74       & 10.26	& 10.03	& 10.07	& 10.12  & 6.58                                                                 & 7.03                                                                       & 7.49                    & 8.03                 & 8.78                \\
JOR                       & 24.01  & 24.91  & 26.08  & 24.9   & 22.96       & -           & 24.93	& 21.9	& 23.54	& 23.46 & 12.86                                                                & 18.61                                                                      & 20.66                   & 20.75                & 29.3                \\
MAU                      & 7.15   & 7.32   & 7.78   & 7.49   & 7.75        & -           & 5.58& 4.32	& 2.25 & 4.05  & 2.75                                                                 & -                                                                          & 6                       & 6.09                 & 6.38                \\
MOR                       & 15.26  & 27.16  & 27.86  & 13.6   & 32.74       & 18.9        & 31.61	& 28.92	& 27.11	& 29.21 & 10.46                                                                & 4.83                                                                       & 12.68                   & 14.27                & 17.02               \\
PAL                       & 26.86  & 26.85  & 29.3   & 29.18  & 29.42       & 12.11       & 20.48	& 18.43	& 22.24	& 20.38 & 14.47                                                                & 16.42                                                                      & 20.41                   & 24.31                & 23.55               \\
UAE                       & 23.17  & 23.53  & 23.57  & 24.93  & 21.22       & 11.78       & 21.18	& 18.92	& 20.9 & 20.33  & 10.93                                                                & -                                                                          & 16.27                   & 18.71                & 19.16               \\
YEM                       & 12.27  & 13.33  & 14.45  & 14.49  & 12.27       & -           & 8.31	& 5.52	& 4.77	& 6.2  & 8.84                                                                 & 11.36                                                                      & 12.95                   & 12.7                 & 11.86               \\
\midrule
\textbf{Average}          & 17.18  & 20.02  & 20.70  & 20.26  & 19.76       & 15.20       & 18.05	& 15.87	& 16.63	& 16.85  & 12.02                                                                & 11.65                                                                      & 16.06                   & 17.42                & 20.58 \\              
\bottomrule
\end{tabular}
}
\caption{\label{blue-main}
Results in BLEU scores. Average is the simple mean of all our varieties. We get three drafts (D1, D2, D2) from Bard, reporting each independently and average scores across the three drafts. NLLB is our supervised baseline with source dialect as MSA. NLLB (Dia) is where the NLLB model is dialect-specific, rather than being an MSA model. SB - supervised baseline, Dia - dialect, Var - varieties, M - model, MST- Microsoft Translation, GT - Google Translate. %\tablecaption
}
\end{table*}







==> Tables/results-tables/bleu-prev.tex <==
\input{emnlp2023-latex/Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & 0-shot & 1-shot & 3-shot & 5-shot & 0-shot      & 5-shot        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 4.99  & 12.04 & 12.36 & 12.58 & 11.65       & 2.36       & 7.56                  & 7.23                                                                 & 11.28                   & 12.13                & 14.87               \\
% MSA                       & 25.53 & 42.92 & 43.1  & 43.66 & 42.06       & 25.28      & 16.42                 & 41.11                                                                & 46.21                   & 47.1                 & 65.74               \\
% ALG                       & 9.85  & 10.92 & 11.74 & 11.78 & 7.46        & -          & 5.24                  & 4.98                                                                 & 6.68                    & 10.15                & 9.13                \\
% EGY                       & 22.68 & 11.26 & 10.8  & 19.94 & 10.05       & 20.74      & 2.89                  & 6.58                                                                 & 7.49                    & 8.03                 & 8.78                \\
% JOR                       & 24.01 & 24.91 & 26.08 & 24.9  & 22.96       & -          & 10.14                 & 12.86                                                                & 20.66                   & 20.75                & 29.3                \\
% MAUR                      & 7.15  & 7.32  & 7.78  & 7.49  & 7.75        & -          & 2.95                  & 2.75                                                                 & 6                       & 6.09                 & 6.38                \\
% MOR                       & 15.26 & 27.16 & 27.86 & 13.6  & 32.74       & 18.9       & 12.69                 & 10.46                                                                & 12.68                   & 14.27                & 17.02               \\
% PAL                       & 26.86 & 26.85 & 29.3  & 29.18 & 29.42       & 12.11      & 11.80                 & 14.47                                                                & 20.41                   & 24.31                & 23.55               \\
% UAE                       & 23.17 & 23.53 & 23.57 & 24.93 & 21.22       & 11.78      & 9.46                  & 10.93                                                                & 16.27                   & 18.71                & 19.16               \\
% YEM                       & 12.27 & 13.33 & 14.45 & 14.49 & 12.27       & -          & 4.93                  & 8.84                                                                 & 12.95                   & 12.7                 & 11.86               \\
% \midrule
% \textbf{Average}          & 17.18 & 20.02 & 20.70 & 20.26 & 19.76       & 15.20      & 8.41                  & 12.02                                                                & 16.06                   & 17.42 & 20.58  \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{blue-main}
% BLEU Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline with source dialect as MSA.  \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}

% % 2nd table with all bard drafts
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                        & 4.99   & 12.04  & 12.36  & 12.58  & 11.65       & 2.36        & 7.96  & 6.99  & 7.72  & 7.56  & 7.23                                                                 & -                                                                          & 11.28                   & 12.13                & 14.87               \\
MSA                       & 25.53  & 42.92  & 43.1   & 43.66  & 42.06       & 25.28       & 18.75 & 15.03 & 15.49 & 16.42 & 41.11                                                                & -                                                                          & 46.21                   & 47.1                 & 65.74               \\
ALG                       & 9.85   & 10.92  & 11.74  & 11.78  & 7.46        & -           & 5.45  & 5.28  & 4.98  & 5.24  & 4.98                                                                 & -                                                                          & 6.68                    & 10.15                & 9.13                \\
EGY                       & 22.68  & 11.26  & 10.8   & 19.94  & 10.05       & 20.74       & 2.97  & 3.05  & 2.66  & 2.89  & 6.58                                                                 & 7.03                                                                       & 7.49                    & 8.03                 & 8.78                \\
JOR                       & 24.01  & 24.91  & 26.08  & 24.9   & 22.96       & -           & 10.98 & 10.21 & 9.23  & 10.14 & 12.86                                                                & 18.61                                                                      & 20.66                   & 20.75                & 29.3                \\
MAU                      & 7.15   & 7.32   & 7.78   & 7.49   & 7.75        & -           & 3.15  & 3.33  & 2.38  & 2.95  & 2.75                                                                 & -                                                                          & 6                       & 6.09                 & 6.38                \\
MOR                       & 15.26  & 27.16  & 27.86  & 13.6   & 32.74       & 18.9        & 13.1  & 12.78 & 12.2  & 12.69 & 10.46                                                                & 4.83                                                                       & 12.68                   & 14.27                & 17.02               \\
PAL                       & 26.86  & 26.85  & 29.3   & 29.18  & 29.42       & 12.11       & 11.72 & 11.26 & 12.41 & 11.80 & 14.47                                                                & 16.42                                                                      & 20.41                   & 24.31                & 23.55               \\
UAE                       & 23.17  & 23.53  & 23.57  & 24.93  & 21.22       & 11.78       & 9.96  & 9.08  & 7     & 9.46  & 10.93                                                                & -                                                                          & 16.27                   & 18.71                & 19.16               \\
YEM                       & 12.27  & 13.33  & 14.45  & 14.49  & 12.27       & -           & 6.1   & 4.93  & 3.76  & 4.93  & 8.84                                                                 & 11.36                                                                      & 12.95                   & 12.7                 & 11.86               \\
\midrule
\textbf{Average}          & 17.18  & 20.02  & 20.70  & 20.26  & 19.76       & 15.20       & 9.01  & 8.19  & 8.02  & 8.41  & 12.02                                                                & 11.65                                                                      & 16.06                   & 17.42                & 20.58 \\              
\bottomrule
\end{tabular}
}
\caption{\label{blue-main}
Results in BLEU scores. \tablecaption
}
\end{table*}







==> Tables/results-tables/chrf++-main.tex <==
\input{Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 23.53  & 38.02  & 37.98  & 38.08  & 38.07       & 9.6        & 32.15                 & 27.02                                                                & 34.56                   & 36.01                & 37.45               \\
% MSA                       & 45.48  & 67.31  & 67.38  & 67.62  & 66.1        & 45.79      & 43.77                 & 63.26                                                                & 68.52                   & 68.28                & 79.06               \\
% ALG                       & 36.41  & 37.48  & 37.99  & 37.99  & 22.78       & -          & 23.55                 & 23.65                                                                & 29.96                   & 35.31                & 31.27               \\
% EGY                       & 46.25  & 43.55  & 43.31  & 44.6   & 42.46       & 45.21      & 22.21                 & 30.09                                                                & 35.7                    & 37.69                & 38.59               \\
% JOR                       & 48.04  & 47.97  & 48.36  & 47.61  & 47.56       & -          & 36.54                 & 33.15                                                                & 43.29                   & 44.82                & 51.15               \\
% MAUR                      & 29.88  & 29.03  & 30.25  & 29.97  & 31.83       & -          & 13.01                 & 19.79                                                                & 26.91                   & 27.44                & 26                  \\
% MOR                       & 30.69  & 48.38  & 48.7   & 29.83  & 52.5        & 34.35      & 37.04                 & 26.36                                                                & 34                      & 34.79                & 38.6                \\
% PAL                       & 50.49  & 49.39  & 50.91  & 50.87  & 51.97       & 29.35      & 34.57                 & 33.95                                                                & 43.69                   & 47.27                & 46.47               \\
% UAE                       & 45.26  & 45.28  & 45.47  & 46.56  & 45.22       & 26.41      & 31.10                 & 28.99                                                                & 36.79                   & 39.83                & 38.81               \\
% YEM                       & 37.42  & 38.1   & 38.59  & 39.02  & 34.7        & -          & 18.95                 & 29.52                                                                & 34.85                   & 36.55                & 35.57               \\
% \midrule
% \textbf{Average}          & 39.35  & 44.45  & 44.89  & 43.22  & 43.32       & 31.79      & 29.29                 & 31.58                                                                & 38.83                   & 40.80                & 42.30      \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{chrf++-main}
% ChrF++ Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline. \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.4}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lcccc|cH|cccc|ccccc}

\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{l}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 23.53  & 38.02  & 37.98  & 38.08  & 38.07       & 9.6         & 36.98 & 35.62 & 37.38 & 36.66 & 27.02                                                                & -                                                                     & 34.56                   & 36.01                & 37.45               \\
MSA                    & 45.48  & 67.31  & 67.38  & 67.62  & 66.1        & 45.79       & 60.34 & 57.69 & 58.19 & 58.74 & 63.26                                                                & -                                                                     & 68.52                   & 68.28                & 79.06               \\
ALG                    & 36.41  & 37.48  & 37.99  & 37.99  & 22.78       & -           & 28.59 & 23.97 & 27.2 & 26.59 & 23.65                                                                & -                                                                     & 29.96                   & 35.31                & 31.27               \\
EGY                    & 46.25  & 43.55  & 43.31  & 44.6   & 42.46       & 45.21       & 38.98 & 37.93 & 39.31 & 38.74 & 30.09                                                                & 33.2                                                                  & 35.7                    & 37.69                & 38.59               \\
JOR                    & 48.04  & 47.97  & 48.36  & 47.61  & 47.56       & -           & 46.61 & 42.1	& 45.34	& 44.68 & 33.15                                                                & 40.04                                                                 & 43.29                   & 44.82                & 51.15               \\
MAU                    & 29.88  & 29.03  & 30.25  & 29.97  & 31.83       & -           & 17.57 & 11.76 & 12.79 & 14.04 & 19.79                                                                & -                                                                     & 26.91                   & 27.44                & 26                  \\
MOR                    & 30.69  & 48.38  & 48.7   & 29.83  & 52.5        & 34.35       & 47.4	& 45.79	& 46.03	& 46.41 & 26.36                                                                & 19.13                                                                 & 34                      & 34.79                & 38.6                \\
PAL                    & 50.49  & 49.39  & 50.91  & 50.87  & 51.97       & 29.35       & 38.98 & 36.85 & 41.7	& 39.18 & 33.95                                                                & 38.46                                                                 & 43.69                   & 47.27                & 46.47               \\
UAE                    & 45.26  & 45.28  & 45.47  & 46.56  & 45.22       & 26.41       & 38.29 & 35.19 & 38.61 & 37.36 & 28.99                                                                & -                                                                     & 36.79                   & 39.83                & 38.81               \\
YEM                    & 37.42  & 38.1   & 38.59  & 39.02  & 34.7        & -           & 23.02 & 18.76 & 19.22 & 20.33 & 29.52                                                                & -                                                                     & 34.85                   & 36.55                & 35.57               \\
\midrule
\textbf{Average}       & 39.35  & 44.45  & 44.89  & 43.22  & 43.32       & 31.79       & 37.68 & 34.57 & 36.58 & 36.27 & 31.58                                                                & 32.54                                                                 & 38.83                   & 40.80                & 42.30       \\
\bottomrule
\end{tabular}
}
\caption{\label{chrf++-main}
Results in ChrF++ Scores. Average is the simple mean of all our varieties. We get three drafts (D1, D2, D2) from Bard, reporting each independently and average scores across the three drafts. NLLB is our supervised baseline with source dialect as MSA. NLLB (Dia) is where the NLLB model is dialect-specific, rather than being an MSA model. SB - supervised baseline, Dia - dialect, Var - varieties, M - model, MST- Microsoft Translation, GT - Google Translate.
}
\end{table*}



==> Tables/results-tables/chrf++-prev.tex <==
\input{emnlp2023-latex/Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 23.53  & 38.02  & 37.98  & 38.08  & 38.07       & 9.6        & 32.15                 & 27.02                                                                & 34.56                   & 36.01                & 37.45               \\
% MSA                       & 45.48  & 67.31  & 67.38  & 67.62  & 66.1        & 45.79      & 43.77                 & 63.26                                                                & 68.52                   & 68.28                & 79.06               \\
% ALG                       & 36.41  & 37.48  & 37.99  & 37.99  & 22.78       & -          & 23.55                 & 23.65                                                                & 29.96                   & 35.31                & 31.27               \\
% EGY                       & 46.25  & 43.55  & 43.31  & 44.6   & 42.46       & 45.21      & 22.21                 & 30.09                                                                & 35.7                    & 37.69                & 38.59               \\
% JOR                       & 48.04  & 47.97  & 48.36  & 47.61  & 47.56       & -          & 36.54                 & 33.15                                                                & 43.29                   & 44.82                & 51.15               \\
% MAUR                      & 29.88  & 29.03  & 30.25  & 29.97  & 31.83       & -          & 13.01                 & 19.79                                                                & 26.91                   & 27.44                & 26                  \\
% MOR                       & 30.69  & 48.38  & 48.7   & 29.83  & 52.5        & 34.35      & 37.04                 & 26.36                                                                & 34                      & 34.79                & 38.6                \\
% PAL                       & 50.49  & 49.39  & 50.91  & 50.87  & 51.97       & 29.35      & 34.57                 & 33.95                                                                & 43.69                   & 47.27                & 46.47               \\
% UAE                       & 45.26  & 45.28  & 45.47  & 46.56  & 45.22       & 26.41      & 31.10                 & 28.99                                                                & 36.79                   & 39.83                & 38.81               \\
% YEM                       & 37.42  & 38.1   & 38.59  & 39.02  & 34.7        & -          & 18.95                 & 29.52                                                                & 34.85                   & 36.55                & 35.57               \\
% \midrule
% \textbf{Average}          & 39.35  & 44.45  & 44.89  & 43.22  & 43.32       & 31.79      & 29.29                 & 31.58                                                                & 38.83                   & 40.80                & 42.30      \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{chrf++-main}
% ChrF++ Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline. \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}

\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 23.53  & 38.02  & 37.98  & 38.08  & 38.07       & 9.6         & 32.44 & 31.48 & 32.53 & 32.15 & 27.02                                                                & -                                                                     & 34.56                   & 36.01                & 37.45               \\
MSA                    & 45.48  & 67.31  & 67.38  & 67.62  & 66.1        & 45.79       & 46.01 & 42.43 & 42.88 & 43.77 & 63.26                                                                & -                                                                     & 68.52                   & 68.28                & 79.06               \\
ALG                    & 36.41  & 37.48  & 37.99  & 37.99  & 22.78       & -           & 24.59 & 21.84 & 24.22 & 23.55 & 23.65                                                                & -                                                                     & 29.96                   & 35.31                & 31.27               \\
EGY                    & 46.25  & 43.55  & 43.31  & 44.6   & 42.46       & 45.21       & 22.58 & 22.33 & 21.71 & 22.21 & 30.09                                                                & 33.2                                                                  & 35.7                    & 37.69                & 38.59               \\
JOR                    & 48.04  & 47.97  & 48.36  & 47.61  & 47.56       & -           & 38.27 & 35.63 & 35.71 & 36.54 & 33.15                                                                & 40.04                                                                 & 43.29                   & 44.82                & 51.15               \\
MAU                    & 29.88  & 29.03  & 30.25  & 29.97  & 31.83       & -           & 15.32 & 11.03 & 12.68 & 13.01 & 19.79                                                                & -                                                                     & 26.91                   & 27.44                & 26                  \\
MOR                    & 30.69  & 48.38  & 48.7   & 29.83  & 52.5        & 34.35       & 37.58 & 36.93 & 36.6  & 37.04 & 26.36                                                                & 19.13                                                                 & 34                      & 34.79                & 38.6                \\
PAL                    & 50.49  & 49.39  & 50.91  & 50.87  & 51.97       & 29.35       & 34.16 & 33.15 & 36.4  & 34.57 & 33.95                                                                & 38.46                                                                 & 43.69                   & 47.27                & 46.47               \\
UAE                    & 45.26  & 45.28  & 45.47  & 46.56  & 45.22       & 26.41       & 32.31 & 29.49 & 31.51 & 31.10 & 28.99                                                                & -                                                                     & 36.79                   & 39.83                & 38.81               \\
YEM                    & 37.42  & 38.1   & 38.59  & 39.02  & 34.7        & -           & 21.08 & 18.14 & 17.63 & 18.95 & 29.52                                                                & -                                                                     & 34.85                   & 36.55                & 35.57               \\
\midrule
\textbf{Average}       & 39.35  & 44.45  & 44.89  & 43.22  & 43.32       & 31.79       & 30.43 & 28.25 & 29.19 & 29.29 & 31.58                                                                & 32.54                                                                 & 38.83                   & 40.80                & 42.30       \\
\bottomrule
\end{tabular}
}
\caption{\label{chrf++-main}
Results in BLEU ChrF++ Scores. \tablecaption
}
\end{table*}



==> Tables/results-tables/chrf-main.tex <==
\input{Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 25.14  & 40.04  & 39.92  & 40     & 40.08       & 9.91       & 33.53                 & 28.25                                                                & 36.28                   & 37.89                & 39.15               \\
% MSA                       & 46.62  & 69.22  & 69.29  & 69.53  & 68.2        & 46.89      & 44.96                 & 65.16                                                                & 70.62                   & 70.11                & 80.28               \\
% ALG                       & 37.91  & 38.98  & 39.53  & 39.43  & 23.32       & -          & 24.02                 & 24.75                                                                & 31.89                   & 37.53                & 32.81               \\
% EGY                       & 47.51  & 45.04  & 44.79  & 45.84  & 44.42       & 46.35      & 22.85                 & 31.78                                                                & 37.29                   & 39.4                 & 40.19               \\
% JOR                       & 48.96  & 48.87  & 49.26  & 48.55  & 49.14       & -          & 37.25                 & 34.38                                                                & 44.63                   & 46.59                & 52.19               \\
% MAUR                      & 31.46  & 30.74  & 31.79  & 31.71  & 33.44       & -          & 13.13                 & 21.36                                                                & 28.76                   & 29.64                & 27.77               \\
% MOR                       & 31.13  & 48.97  & 49.24  & 30.31  & 52.96       & 34.71      & 37.13                 & 27.25                                                                & 34.79                   & 35.53                & 39.38               \\
% PAL                       & 51.65  & 50.61  & 52.05  & 51.98  & 53.17       & 30.08      & 35.21                 & 35.4                                                                 & 45.24                   & 48.96                & 48.02               \\
% UAE                       & 46.06  & 46.27  & 46.41  & 47.43  & 47.05       & 26.97      & 31.51                 & 29.92                                                                & 37.68                   & 41.1                 & 39.79               \\
% YEM                       & 38.88  & 39.45  & 39.89  & 40.38  & 35.97       & -          & 19.26                 & 30.99                                                                & 35.86                   & 37.94                & 36.88               \\
% \midrule
% \textbf{Average}          & 40.53  & 45.82  & 46.22  & 44.52  & 44.78       & 32.49      & 29.89                 & 32.92                                                                & 40.30                   & 42.47                & 43.65   \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{chrf-main}
% ChrF Scores. ChrF Scores. \tablecaption
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.5}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 25.14  & 40.04  & 39.92  & 40     & 40.08       & 9.91        & 38.53 & 37.32 & 38.92 & 38.26 & 28.25                                                                & -                                                                     & 36.28                   & 37.89                & 39.15               \\
MSA                    & 46.62  & 69.22  & 69.29  & 69.53  & 68.2        & 46.89       & 62.7	& 60.09	& 60.5 & 61.1 & 65.16                                                                & -                                                                     & 70.62                   & 70.11                & 80.28               \\
ALG                    & 37.91  & 38.98  & 39.53  & 39.43  & 23.32       & -           & 29.51 & 24.73 & 28.04 & 27.43 & 24.75                                                                & -                                                                     & 31.89                   & 37.53                & 32.81               \\
EGY                    & 47.51  & 45.04  & 44.79  & 45.84  & 44.42       & 46.35       & 40.11 & 38.99 & 40.5	& 39.87 & 31.78                                                                & 34.79                                                                 & 37.29                   & 39.4                 & 40.19               \\
JOR                    & 48.96  & 48.87  & 49.26  & 48.55  & 49.14       & -           & 47.52 & 42.92 & 46.26 & 45.57 & 34.38                                                                & 41.19                                                                 & 44.63                   & 46.59                & 52.19               \\
MAU                    & 31.46  & 30.74  & 31.79  & 31.71  & 33.44       & -           & 18.08 & 11.84 & 13.12 & 14.35 & 21.36                                                                & -                                                                     & 28.76                   & 29.64                & 27.77               \\
MOR                    & 31.13  & 48.97  & 49.24  & 30.31  & 52.96       & 34.71       & 47.52 & 46.03 & 46.24 & 46.6 & 27.25                                                                & 20.55                                                                 & 34.79                   & 35.53                & 39.38               \\
PAL                    & 51.65  & 50.61  & 52.05  & 51.98  & 53.17       & 30.08       & 40.16 & 38.12 & 42.96 & 40.41 & 35.4                                                                 & 39.73                                                                 & 45.24                   & 48.96                & 48.02               \\
UAE                    & 46.06  & 46.27  & 46.41  & 47.43  & 47.05       & 26.97       & 38.82 & 35.76 & 39.29 & 37.96 & 29.92                                                                & -                                                                     & 37.68                   & 41.1                 & 39.79               \\
YEM                    & 38.88  & 39.45  & 39.89  & 40.38  & 35.97       & -           & 23.57 & 19.07 & 19.6	& 20.75 & 30.99                                                                & 33.65                                                                 & 35.86                   & 37.94                & 36.88               \\
\midrule
\textbf{Average}       & 40.53  & 45.82  & 46.22  & 44.52  & 44.78       & 32.49       & 38.65 & 35.49 & 37.54 & 37.23 & 32.92                                                                & 33.98      \\              
\bottomrule
\end{tabular}
}
\caption{\label{chrf-appendix}
ChrF Scores. Average is the simple mean of all our varieties. We get three drafts (D1, D2, D2) from Bard, reporting each independently and average scores across the three drafts. NLLB is our supervised baseline with source dialect as MSA. NLLB (Dia) is where the NLLB model is dialect-specific, rather than being an MSA model. SB - supervised baseline, Dia - dialect, Var - varieties, M - model, MST- Microsoft Translation, GT - Google Translate.
}
\end{table*}


==> Tables/results-tables/chrf-prev.tex <==
\input{emnlp2023-latex/Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 25.14  & 40.04  & 39.92  & 40     & 40.08       & 9.91       & 33.53                 & 28.25                                                                & 36.28                   & 37.89                & 39.15               \\
% MSA                       & 46.62  & 69.22  & 69.29  & 69.53  & 68.2        & 46.89      & 44.96                 & 65.16                                                                & 70.62                   & 70.11                & 80.28               \\
% ALG                       & 37.91  & 38.98  & 39.53  & 39.43  & 23.32       & -          & 24.02                 & 24.75                                                                & 31.89                   & 37.53                & 32.81               \\
% EGY                       & 47.51  & 45.04  & 44.79  & 45.84  & 44.42       & 46.35      & 22.85                 & 31.78                                                                & 37.29                   & 39.4                 & 40.19               \\
% JOR                       & 48.96  & 48.87  & 49.26  & 48.55  & 49.14       & -          & 37.25                 & 34.38                                                                & 44.63                   & 46.59                & 52.19               \\
% MAUR                      & 31.46  & 30.74  & 31.79  & 31.71  & 33.44       & -          & 13.13                 & 21.36                                                                & 28.76                   & 29.64                & 27.77               \\
% MOR                       & 31.13  & 48.97  & 49.24  & 30.31  & 52.96       & 34.71      & 37.13                 & 27.25                                                                & 34.79                   & 35.53                & 39.38               \\
% PAL                       & 51.65  & 50.61  & 52.05  & 51.98  & 53.17       & 30.08      & 35.21                 & 35.4                                                                 & 45.24                   & 48.96                & 48.02               \\
% UAE                       & 46.06  & 46.27  & 46.41  & 47.43  & 47.05       & 26.97      & 31.51                 & 29.92                                                                & 37.68                   & 41.1                 & 39.79               \\
% YEM                       & 38.88  & 39.45  & 39.89  & 40.38  & 35.97       & -          & 19.26                 & 30.99                                                                & 35.86                   & 37.94                & 36.88               \\
% \midrule
% \textbf{Average}          & 40.53  & 45.82  & 46.22  & 44.52  & 44.78       & 32.49      & 29.89                 & 32.92                                                                & 40.30                   & 42.47                & 43.65   \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{chrf-main}
% ChrF Scores. ChrF Scores. \tablecaption
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 25.14  & 40.04  & 39.92  & 40     & 40.08       & 9.91        & 33.77 & 32.95 & 33.86 & 33.53 & 28.25                                                                & -                                                                     & 36.28                   & 37.89                & 39.15               \\
MSA                    & 46.62  & 69.22  & 69.29  & 69.53  & 68.2        & 46.89       & 47.19 & 43.65 & 44.05 & 44.96 & 65.16                                                                & -                                                                     & 70.62                   & 70.11                & 80.28               \\
ALG                    & 37.91  & 38.98  & 39.53  & 39.43  & 23.32       & -           & 25.08 & 22.25 & 24.73 & 24.02 & 24.75                                                                & -                                                                     & 31.89                   & 37.53                & 32.81               \\
EGY                    & 47.51  & 45.04  & 44.79  & 45.84  & 44.42       & 46.35       & 23.24 & 22.95 & 22.36 & 22.85 & 31.78                                                                & 34.79                                                                 & 37.29                   & 39.4                 & 40.19               \\
JOR                    & 48.96  & 48.87  & 49.26  & 48.55  & 49.14       & -           & 38.98 & 36.34 & 36.44 & 37.25 & 34.38                                                                & 41.19                                                                 & 44.63                   & 46.59                & 52.19               \\
MAU                    & 31.46  & 30.74  & 31.79  & 31.71  & 33.44       & -           & 15.52 & 10.99 & 12.87 & 13.13 & 21.36                                                                & -                                                                     & 28.76                   & 29.64                & 27.77               \\
MOR                    & 31.13  & 48.97  & 49.24  & 30.31  & 52.96       & 34.71       & 37.63 & 37.03 & 36.72 & 37.13 & 27.25                                                                & 20.55                                                                 & 34.79                   & 35.53                & 39.38               \\
PAL                    & 51.65  & 50.61  & 52.05  & 51.98  & 53.17       & 30.08       & 34.74 & 33.86 & 37.03 & 35.21 & 35.4                                                                 & 39.73                                                                 & 45.24                   & 48.96                & 48.02               \\
UAE                    & 46.06  & 46.27  & 46.41  & 47.43  & 47.05       & 26.97       & 32.69 & 29.85 & 31.99 & 31.51 & 29.92                                                                & -                                                                     & 37.68                   & 41.1                 & 39.79               \\
YEM                    & 38.88  & 39.45  & 39.89  & 40.38  & 35.97       & -           & 21.49 & 18.39 & 17.91 & 19.26 & 30.99                                                                & 33.65                                                                 & 35.86                   & 37.94                & 36.88               \\
\midrule
\textbf{Average}       & 40.53  & 45.82  & 46.22  & 44.52  & 44.78       & 32.49       & 31.03 & 28.83 & 29.80 & 29.89 & 32.92                                                                & 33.98      \\              
\bottomrule
\end{tabular}
}
\caption{\label{chrf-appendix}
ChrF Scores. \tablecaption
}
\end{table*}


==> Tables/results-tables/comet-main.tex <==
\input{Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & 0-shot & 1-shot & 3-shot & 5-shot & 0-shot      & 5-shot        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 4.99  & 12.04 & 12.36 & 12.58 & 11.65       & 2.36       & 7.56                  & 7.23                                                                 & 11.28                   & 12.13                & 14.87               \\
% MSA                       & 25.53 & 42.92 & 43.1  & 43.66 & 42.06       & 25.28      & 16.42                 & 41.11                                                                & 46.21                   & 47.1                 & 65.74               \\
% ALG                       & 9.85  & 10.92 & 11.74 & 11.78 & 7.46        & -          & 5.24                  & 4.98                                                                 & 6.68                    & 10.15                & 9.13                \\
% EGY                       & 22.68 & 11.26 & 10.8  & 19.94 & 10.05       & 20.74      & 2.89                  & 6.58                                                                 & 7.49                    & 8.03                 & 8.78                \\
% JOR                       & 24.01 & 24.91 & 26.08 & 24.9  & 22.96       & -          & 10.14                 & 12.86                                                                & 20.66                   & 20.75                & 29.3                \\
% MAUR                      & 7.15  & 7.32  & 7.78  & 7.49  & 7.75        & -          & 2.95                  & 2.75                                                                 & 6                       & 6.09                 & 6.38                \\
% MOR                       & 15.26 & 27.16 & 27.86 & 13.6  & 32.74       & 18.9       & 12.69                 & 10.46                                                                & 12.68                   & 14.27                & 17.02               \\
% PAL                       & 26.86 & 26.85 & 29.3  & 29.18 & 29.42       & 12.11      & 11.80                 & 14.47                                                                & 20.41                   & 24.31                & 23.55               \\
% UAE                       & 23.17 & 23.53 & 23.57 & 24.93 & 21.22       & 11.78      & 9.46                  & 10.93                                                                & 16.27                   & 18.71                & 19.16               \\
% YEM                       & 12.27 & 13.33 & 14.45 & 14.49 & 12.27       & -          & 4.93                  & 8.84                                                                 & 12.95                   & 12.7                 & 11.86               \\
% \midrule
% \textbf{Average}          & 17.18 & 20.02 & 20.70 & 20.26 & 19.76       & 15.20      & 8.41                  & 12.02                                                                & 16.06                   & 17.42 & 20.58  \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{blue-main}
% BLEU Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline with source dialect as MSA.  \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}

% % 2nd table with all bard drafts
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.4}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{llccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Metrics}} & \multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}                                  & \multicolumn{2}{c}{\textbf{GPT4}}                     & \multicolumn{4}{c}{\textbf{Bard}}                      & \textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MS}} & \multirow{2}{*}{\textbf{GT}} \\
                                  &                                 & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot} & \multicolumn{1}{l}{\textbf{5-shot}} & \textbf{D1} & \textbf{D2} & \textbf{D3} & \textbf{Avg} &                                                              &                                                               &                                  &                              &                              \\
\midrule
\multirow{11}{*}{BLEU}            & CA                              & 11.2            & 12.04           & 12.36           & 12.58           & 11.67           & 11.08                               & 12.25       & 10.37       & 12.36       & 11.66        & 7.23                                                         & -                                                             & 11.28                            & 12.13                        & 14.87                        \\
                                  & MSA                             & 42.4            & 43.57           & 43.72           & 44.28           & 42.46           & 43.2                                & 37.02       & 32.98       & 35.73       & 35.24        & 41.3                                                         & -                                                             & 46.55                            & 47.32                        & 66.12                        \\
                                  & ALG                             & 9.78            & 11.17           & 12              & 12.18           & 7.89            & 12.28                               & 9.25        & 7.34        & 7.66        & 8.08         & 4.85                                                         & -                                                             & 6.78                             & 10.03                        & 9.09                         \\
                                  & EGY                             & 10.03           & 11.26           & 10.8            & 10.99           & 10.05           & 10.06                               & 10.26       & 10.03       & 10.07       & 10.12        & 6.58                                                         & -                                                             & 7.49                             & 8.03                         & 8.78                         \\
                                  & JOR                             & 24.01           & 24.91           & 26.08           & 24.9            & 22.96           & -                                   & 24.93       & 21.9        & 23.54       & 23.46        & 12.86                                                        & -                                                             & 20.66                            & 20.75                        & 29.3                         \\
                                  & MAUR                            & 7.17            & 7.33            & 7.73            & 7.55            & 7.77            & 8.13                                & 5.51        & 4.25        & 2.23        & 4.00         & 2.77                                                         & -                                                             & 6.18                             & 6.11                         & 6.58                         \\
                                  & MOR                             & 27.02           & 28.03           & 28.84           & 28.7            & 32.74           & 33.08                               & 31.7        & 29.05       & 27.22       & 29.32        & 10.46                                                        & -                                                             & 12.68                            & 14.27                        & 17.02                        \\
                                  & PAL                             & 26.86           & 26.85           & 29.3            & 29.18           & 29.42           & 28.19                               & 20.48       & 18.43       & 22.24       & 20.38        & 14.47                                                        & -                                                             & 20.41                            & 24.31                        & 23.55                        \\
                                  & UAE                             & 23.29           & 23.76           & 23.82           & 25.23           & 21.5            & 26.4                                & 21.26       & 19.01       & 21.02       & 20.43        & 11.01                                                        & -                                                             & 16.35                            & 18.81                        & 19.28                        \\
                                  & YEM                             & 12.3            & 13.46           & 14.65           & 14.66           & 12.46           & 6.02                                & 8.3         & 5.51        & 4.76        & 6.19         & 8.89                                                         & -                                                             & 13.03                            & 12.7                         & 12.02                        \\ \cline{2-17}
                                  & \textbf{Avg}                    & 19.41           & 20.24           & 20.93           & 21.03           & 19.89           & 19.83                               & 18.10       & 15.89       & 16.68       & 16.89        & 12.04                                                        & -                                                             & 16.14                            & 17.45                        & 20.66                        \\
\midrule
\multirow{11}{*}{COMET}           & CA                              & 48.53           & 69.87           & 69.84           & 70.02           & 70.84           & 70.72                               & 59.37       & 57.56       & 59.2        & 58.71        & 58.31                                                        & -                                                             & 63.01                            & 62.77                        & 66.08                        \\
                                  & MSA                             & 76.99           & 86.03           & 86.12           & 86.14           & 86.06           & 86.09                               & 61.99       & 61.48       & 61.35       & 61.61        & 84.71                                                        & -                                                             & 86.05                            & 85.67                        & 87.33                        \\
                                  & ALG                             & 79.65           & 80.13           & 80.23           & 80.19           & 72.83           & -                                   & 73.04       & 71.99       & 72.56       & 72.53        & 73.75                                                        & -                                                             & 75.91                            & 77.35                        & -                            \\
                                  & EGY                             & 86.27           & 56.58           & 57.02           & 86.02           & 57.52           & 57.81                               & 55.85       & 43.29       & 42.23       & 47.12        & 49.52                                                        & -                                                             & 51.02                            & 53.16                        & 54.42                        \\
                                  & JOR                             & 73.96           & 74.69           & 75.03           & 74.68           & 75.8            & -                                   & 48.19       & 48.7        & 47.71       & 48.20        & 60.28                                                        & -                                                             & 67                               & 70.04                        & 71.79                        \\
                                  & MAUR                            & 57.48           & 58.12           & 59.45           & 59.88           & 58.12           & -                                   & 43.98       & 41.23       & 42.36       & 42.52        & 48.22                                                        & -                                                             & 51.99                            & 50.92                        & 51.11                        \\
                                  & MOR                             & 70.05           & 69.54           & 70.48           & 50.62           & 73.92           & 73.85                               & 72.15       & 70.53       & 71.61       & 71.43        & 53.2                                                         & -                                                             & 54.45                            & 51.87                        & 56.51                        \\
                                  & PAL                             & 73.56           & 73.88           & 74.35           & 74.45           & 76.28           & 67.67                               & 52.1        & 52.44       & 52.08       & 52.21        & 60.62                                                        & -                                                             & 66.02                            & 68.98                        & 68.79                        \\
                                  & UAE                             & 69.16           & 69.18           & 69.41           & 70.41           & 72.11           & 62.48                               & 48.11       & 47.55       & 47.66       & 47.77        & 54.48                                                        & -                                                             & 59.13                            & 61.33                        & 61.17                        \\
                                  & YEM                             & 63.94           & 64.47           & 65.33           & 64.87           & 61.76           & -                                   & 55.81       & 52.63       & 54.62       & 54.35        & 56.61                                                        & -                                                             & 60.85                            & 61.31                        & 60.96                        \\ \cline{2-17}
                                  & \textbf{Avg}                    & 69.96           & 70.25           & 70.73           & 71.73           & 70.52           & 69.77                               & 57.06       & 54.74       & 55.14       & 55.65        & 59.97                                                        & -                                                             & 63.54                            & 64.34                        & 64.24                        \\
\midrule
\multirow{11}{*}{ChrF++}          & CA                              & 37.71           & 38.02           & 37.98           & 38.08           & 37.99           & 37.04                               & 36.98       & 35.62       & 37.38       & 36.66        & 27.02                                                        & -                                                             & 34.56                            & 36.01                        & 37.45                        \\
                                  & MSA                             & 67.26           & 67.7            & 67.75           & 68              & 66.36           & 67.29                               & 60.55       & 57.78       & 58.3        & 58.88        & 63.37                                                        & -                                                             & 68.81                            & 68.54                        & 79.27                        \\
                                  & ALG                             & 35.98           & 37.2            & 37.7            & 37.75           & 22.75           & 38.92                               & 27.98       & 23.29       & 26.63       & 25.97        & 22.97                                                        & -                                                             & 29.67                            & 34.87                        & 30.99                        \\
                                  & EGY                             & 41.94           & 43.55           & 43.31           & 43.3            & 42.46           & 41.48                               & 38.98       & 37.93       & 39.31       & 38.74        & 30.09                                                        & -                                                             & 35.7                             & 37.69                        & 38.59                        \\
                                  & JOR                             & 48.04           & 47.97           & 48.36           & 47.61           & 47.56           & 47.47                               & 46.61       & 42.1        & 45.34       & 44.68        & 33.15                                                        & -                                                             & 43.29                            & 44.82                        & 51.15                        \\
                                  & MAUR                            & 29.97           & 29.01           & 30.2            & 30.01           & 31.92           & 31.14                               & 17.57       & 11.73       & 12.8        & 14.03        & 19.81                                                        & -                                                             & 27.14                            & 27.51                        & 26.18                        \\
                                  & MOR                             & 47.61           & 48.59           & 48.92           & 49.09           & 52.5            & 53.01                               & 47.47       & 45.81       & 46.07       & 46.45        & 26.36                                                        & -                                                             & 34                               & 34.79                        & 38.6                         \\
                                  & PAL                             & 50.49           & 49.39           & 50.91           & 50.87           & 51.97           & 51.36                               & 38.98       & 36.85       & 41.7        & 39.18        & 33.95                                                        & -                                                             & 43.69                            & 47.27                        & 46.47                        \\
                                  & UAE                             & 45.25           & 45.38           & 45.59           & 46.72           & 45.4            & 47.1                                & 38.31       & 35.26       & 38.68       & 37.42        & 29.01                                                        & -                                                             & 36.89                            & 39.9                         & 38.85                        \\
                                  & YEM                             & 37.48           & 38.22           & 38.71           & 39.15           & 34.85           & 20.94                               & 23.12       & 18.85       & 19.29       & 20.42        & 29.58                                                        & -                                                             & 34.97                            & 36.59                        & 35.73                        \\ \cline{2-17}
                                  & \textbf{Avg}                    & 44.17           & 44.50           & 44.94           & 45.06           & 43.38           & 43.58                               & 37.66       & 34.52       & 36.55       & 36.24        & 31.53                                                        & -                                                             & 38.87                            & 40.80                        & 42.33       \\

\bottomrule
\end{tabular}
}

\caption{\label{blue-main}
Results in COMET scores. Average is the simple mean of all our varieties. We get three drafts (D1, D2, D2) from Bard, reporting each independently and average scores across the three drafts. NLLB is our supervised baseline with source dialect as MSA. NLLB (Dia) is where the NLLB model is dialect-specific, rather than being an MSA model. SB - supervised baseline, Dia - dialect, Var - varieties, M - model, MST- Microsoft Translation, GT - Google Translate. %\tablecaption
}
\end{table*}







==> Tables/results-tables/nllb-dialectal.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.0}   %to squeeze table content
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{lccccc}

\toprule
Task-DA & NLLB-DA & BLEU  & ChrF  & ChrF++ & TER    \\
\midrule
EGY     & EGY     & 7.03  & 34.79 & 33.2   & 186.52 \\
JOR     & S. LEV  & 18.61 & 41.19 & 40.04  & 82.14  \\
MOR     & MOR     & 4.83  & 20.55 & 19.13  & 103.66 \\
PAL     & S. LEV  & 16.42 & 39.73 & 38.46  & 77.19  \\
YEM     & TA      & 11.36 & 33.65 & 32.54  & 91.48 \\

\bottomrule

\end{tabular}
}
\caption{\label{nllb-dialectal}
NLLB Dialectal Result. S. LEV is South Levantine. TA is Taizzi Adeni.
}
\end{table}

==> Tables/results-tables/ter-main.tex <==
\input{Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 93.91  & 84.5   & 83.65  & 83.69  & 85.85       & 96.03      & 153.15                & 90.04                                                                & 82                      & 84.08                & 84.1                \\
% MSA                       & 63.91  & 45.14  & 44.78  & 44.26  & 45.89       & 62.52      & 196.30                & 45.63                                                                & 41.73                   & 40.61                & 28.95               \\
% ALG                       & 91.19  & 84.45  & 83.96  & 82.16  & 89.08       & -          & 182.45                & 122.56                                                               & 92.61                   & 86.42                & 89.58               \\
% EGY                       & 68.18  & 172.43 & 174.6  & 72.79  & 174.76      & 68.62      & 694.50                & 173.64                                                               & 181.98                  & 180.38               & 169.82              \\
% JOR                       & 73.03  & 70.25  & 68.28  & 69.98  & 73.03       & -          & 218.27                & 109.68                                                               & 74.75                   & 73.33                & 66.87               \\
% MAUR                      & 107.01 & 99.21  & 99.11  & 98.71  & 103.62      & -          & 212.84                & 132.76                                                               & 100.63                  & 101.39               & 102.44              \\
% MOR                       & 79.01  & 65.93  & 65.55  & 79.01  & 56.33       & 74.45      & 204.33                & 100.02                                                               & 82.52                   & 80.57                & 77.62               \\
% PAL                       & 61.89  & 61.57  & 58.7   & 58.79  & 56.47       & 77.94      & 168.95                & 86.12                                                                & 67.42                   & 61.72                & 66.37               \\
% UAE                       & 72.62  & 70.03  & 70.42  & 67.65  & 82.58       & 86.44      & 202.86                & 85.59                                                                & 78.2                    & 74.99                & 76.85               \\
% YEM                       & 88.96  & 86.43  & 83.61  & 85.41  & 88.72       & -          & 180.96                & 88.03                                                                & 84.12                   & 83.91                & 87.57               \\
% \midrule
% \textbf{Average}          & 79.97  & 83.99  & 83.27  & 74.25  & 85.63       & 77.67      & 241.46                & 103.41                                                               & 88.60                   & 86.74                & 85.02           \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{ter-main}
% TER Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline. \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.5}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 93.91  & 84.5   & 83.65  & 83.69  & 85.85       & 96.03       & 87.89 & 102.66 & 88.07 & 92.87 & 90.04                                                                &                                                                       & 82                      & 84.08                & 84.1                \\
MSA                    & 63.91  & 45.14  & 44.78  & 44.26  & 45.89       & 62.52       & 56.41 & 69.49 & 64.76 & 63.55 & 45.63                                                                &                                                                       & 41.73                   & 40.61                & 28.95               \\
ALG                    & 91.19  & 84.45  & 83.96  & 82.16  & 89.08       & -           & 97.26 & 112.86 & 119.75 & 109.96 & 122.56                                                               &                                                                       & 92.61                   & 86.42                & 89.58               \\
EGY                    & 68.18  & 172.43 & 174.6  & 72.79  & 174.76      & 68.62       & 171.15 & 176.4 & 176.61 & 174.72 & 173.64                                                               & 186.52                                                                & 181.98                  & 180.38               & 169.82              \\
JOR                    & 73.03  & 70.25  & 68.28  & 69.98  & 73.03       & -           & 70.91 & 76.55 & 71.9	& 73.12 & 109.68                                                               & 82.14                                                                 & 74.75                   & 73.33                & 66.87               \\
MAU                    & 107.01 & 99.21  & 99.11  & 98.71  & 103.62      & -           & 109.62 & 105.84 & 251.81	& 155.76 & 132.76                                                               &                                                                       & 100.63                  & 101.39               & 102.44              \\
MOR                    & 79.01  & 65.93  & 65.55  & 79.01  & 56.33       & 74.45       & 62.19 & 68.93 & 76.28 & 69.13 & 100.02                                                               & 103.66                                                                & 82.52                   & 80.57                & 77.62               \\
PAL                    & 61.89  & 61.57  & 58.7   & 58.79  & 56.47       & 77.94       & 74.59 & 77.34 & 67.96 & 73.3 & 86.12                                                                & 77.19                                                                 & 67.42                   & 61.72                & 66.37               \\
UAE                    & 72.62  & 70.03  & 70.42  & 67.65  & 82.58       & 86.44       & 81.09 & 77.78 & 74.77 & 77.88 & 85.59                                                                &                                                                       & 78.2                    & 74.99                & 76.85               \\
YEM                    & 88.96  & 86.43  & 83.61  & 85.41  & 88.72       & -           & 111.57 & 154.7 & 185.75 & 150.67 & 88.03                                                                & 91.48                                                                 & 84.12                   & 83.91                & 87.57               \\
\midrule
\textbf{Average}       & 79.97  & 83.99  & 83.27  & 74.25  & 85.63       & 77.67       & 92.27 & 102.26 & 117.77 & 104.1 & 103.41                                                               & 108.20                                                                & 88.60                   & 86.74                & 85.02  \\              
\bottomrule
\end{tabular}
}
\caption{\label{ter-appendix}
TER Scores. Average is the simple mean of all our varieties. We get three drafts (D1, D2, D2) from Bard, reporting each independently and average scores across the three drafts. NLLB is our supervised baseline with source dialect as MSA. NLLB (Dia) is where the NLLB model is dialect-specific, rather than being an MSA model. SB - supervised baseline, Dia - dialect, Var - varieties, M - model, MST- Microsoft Translation, GT - Google Translate.
}
\end{table*}

==> Tables/results-tables/ter-prev.tex <==
\input{emnlp2023-latex/Tables/results-tables/table-caption}
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table*}[]
% \centering
% \footnotesize 
% \renewcommand{\arraystretch}{1.}   %to squeeze table content
% \resizebox{0.95\linewidth}{!}{%
% % \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
% \begin{tabular}{lccccccccccc}
% \toprule
% \multirow{2}{*}{TD/Model} & \multicolumn{4}{c}{ChatGPT}   & \multicolumn{2}{c}{GPT4} & \multirow{2}{*}{Bard} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}} & \multirow{2}{*}{Amazon} & \multirow{2}{*}{Microsoft} & \multirow{2}{*}{Google} \\

%                           & shot-0   & shot-1   & shot-3   & shot-5   & shot-0         & shot-5        &                       &                                                                      &                         &                      &                     \\
% \midrule
% CA                        & 93.91  & 84.5   & 83.65  & 83.69  & 85.85       & 96.03      & 153.15                & 90.04                                                                & 82                      & 84.08                & 84.1                \\
% MSA                       & 63.91  & 45.14  & 44.78  & 44.26  & 45.89       & 62.52      & 196.30                & 45.63                                                                & 41.73                   & 40.61                & 28.95               \\
% ALG                       & 91.19  & 84.45  & 83.96  & 82.16  & 89.08       & -          & 182.45                & 122.56                                                               & 92.61                   & 86.42                & 89.58               \\
% EGY                       & 68.18  & 172.43 & 174.6  & 72.79  & 174.76      & 68.62      & 694.50                & 173.64                                                               & 181.98                  & 180.38               & 169.82              \\
% JOR                       & 73.03  & 70.25  & 68.28  & 69.98  & 73.03       & -          & 218.27                & 109.68                                                               & 74.75                   & 73.33                & 66.87               \\
% MAUR                      & 107.01 & 99.21  & 99.11  & 98.71  & 103.62      & -          & 212.84                & 132.76                                                               & 100.63                  & 101.39               & 102.44              \\
% MOR                       & 79.01  & 65.93  & 65.55  & 79.01  & 56.33       & 74.45      & 204.33                & 100.02                                                               & 82.52                   & 80.57                & 77.62               \\
% PAL                       & 61.89  & 61.57  & 58.7   & 58.79  & 56.47       & 77.94      & 168.95                & 86.12                                                                & 67.42                   & 61.72                & 66.37               \\
% UAE                       & 72.62  & 70.03  & 70.42  & 67.65  & 82.58       & 86.44      & 202.86                & 85.59                                                                & 78.2                    & 74.99                & 76.85               \\
% YEM                       & 88.96  & 86.43  & 83.61  & 85.41  & 88.72       & -          & 180.96                & 88.03                                                                & 84.12                   & 83.91                & 87.57               \\
% \midrule
% \textbf{Average}          & 79.97  & 83.99  & 83.27  & 74.25  & 85.63       & 77.67      & 241.46                & 103.41                                                               & 88.60                   & 86.74                & 85.02           \\
% \bottomrule
% \end{tabular}
% }
% \caption{\label{ter-main}
% TER Scores. Average is the simple mean across the $10$ varieties. We get three drafts from Bard and we report average scores. NLLB is our supervised baseline. \textcolor{red}{Abdul: Please write a good and detailed caption.}
% }
% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\footnotesize 
\renewcommand{\arraystretch}{1.}   %to squeeze table content
\resizebox{1.0\linewidth}{!}{%
% \begin{tabular}{l:cccc:cc:c:c:ccc} # dashed line looks ugly
\begin{tabular}{lccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Var/M}} & \multicolumn{4}{c}{\textbf{ChatGPT}}       & \multicolumn{2}{c}{\textbf{GPT-4}} & \multicolumn{4}{c}{\textbf{Bard}}      & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (SB)\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}NLLB\\ (Dia)\end{tabular}}} & \multirow{2}{*}{\textbf{Amazon}} & \multirow{2}{*}{\textbf{MST}} & \multirow{2}{*}{\textbf{GT}} \\
                          & \textbf{0-shot} & \textbf{1-shot} & \textbf{3-shot} & \textbf{5-shot} & \textbf{0-shot}      & \textbf{5-shot}      & \textbf{D1}    & \textbf{D2}    & \textbf{D3}    & \textbf{Avg}   &                                                                      &                                                                            &                         &                      &                     \\

\midrule
CA                     & 93.91  & 84.5   & 83.65  & 83.69  & 85.85       & 96.03       & 144.3  & 161.97 & 153.19 & 153.15 & 90.04                                                                &                                                                       & 82                      & 84.08                & 84.1                \\
MSA                    & 63.91  & 45.14  & 44.78  & 44.26  & 45.89       & 62.52       & 167.02 & 214.56 & 207.32 & 196.30 & 45.63                                                                &                                                                       & 41.73                   & 40.61                & 28.95               \\
ALG                    & 91.19  & 84.45  & 83.96  & 82.16  & 89.08       & -           & 185.42 & 162.86 & 199.08 & 182.45 & 122.56                                                               &                                                                       & 92.61                   & 86.42                & 89.58               \\
EGY                    & 68.18  & 172.43 & 174.6  & 72.79  & 174.76      & 68.62       & 665.97 & 654.9  & 762.64 & 694.50 & 173.64                                                               & 186.52                                                                & 181.98                  & 180.38               & 169.82              \\
JOR                    & 73.03  & 70.25  & 68.28  & 69.98  & 73.03       & -           & 212.36 & 200.59 & 241.87 & 218.27 & 109.68                                                               & 82.14                                                                 & 74.75                   & 73.33                & 66.87               \\
MAU                    & 107.01 & 99.21  & 99.11  & 98.71  & 103.62      & -           & 205.14 & 162.26 & 271.13 & 212.84 & 132.76                                                               &                                                                       & 100.63                  & 101.39               & 102.44              \\
MOR                    & 79.01  & 65.93  & 65.55  & 79.01  & 56.33       & 74.45       & 199.3  & 200.38 & 213.3  & 204.33 & 100.02                                                               & 103.66                                                                & 82.52                   & 80.57                & 77.62               \\
PAL                    & 61.89  & 61.57  & 58.7   & 58.79  & 56.47       & 77.94       & 169.87 & 165.76 & 171.21 & 168.95 & 86.12                                                                & 77.19                                                                 & 67.42                   & 61.72                & 66.37               \\
UAE                    & 72.62  & 70.03  & 70.42  & 67.65  & 82.58       & 86.44       & 204.11 & 197.75 & 206.73 & 202.86 & 85.59                                                                &                                                                       & 78.2                    & 74.99                & 76.85               \\
YEM                    & 88.96  & 86.43  & 83.61  & 85.41  & 88.72       & -           & 145.91 & 168.67 & 228.29 & 180.96 & 88.03                                                                & 91.48                                                                 & 84.12                   & 83.91                & 87.57               \\
\midrule
\textbf{Average}       & 79.97  & 83.99  & 83.27  & 74.25  & 85.63       & 77.67       & 229.94 & 228.97 & 265.48 & 241.46 & 103.41                                                               & 108.20                                                                & 88.60                   & 86.74                & 85.02  \\              
\bottomrule
\end{tabular}
}
\caption{\label{ter-appendix}
TER Scores. \tablecaption
}
\end{table*}
